Adaptive Subband Compression for Streaming of Continuous Point-on-Wave and PMU Data

A data compression system capable of providing real-time streaming of high-resolution continuous point-on-wave (CPOW) and phasor measurement unit (PMU) measurements is proposed. Referred to as adaptive subband compression (ASBC), the proposed technique partitions the signal space into subbands and adaptively compresses subband signals based on each subband's active bandwidth. The proposed technique conforms to existing industry phasor measurement standards, making it suitable for streaming high-resolution CPOW and PMU data either in continuous or burst on-demand/event-triggered modes. Experiments on synthetic and real data show that ASBC reduces the CPOW sampling rates by several orders of magnitude for real-time streaming while maintaining the precision required by industry standards.

==> Decode_v1.tex <==


ASBC decoders are located at regional data concentrators or the control center where compressed streaming data are reconstructed.
Fig.~\ref{fig:decode} illustrates the schematic of an ASBC decoder.  The functionalities of individual components are explained below.

The de-multiplexing block is the inverse of the multiplexing block at the encoder.  It parses the single bit-stream into subband data streams $\tilde{x}^Q_k$ and $\tilde{x}_e^Q$  sent by the transmitter.

The decompression block reverses the compression block and
generates estimated harmonics  (in baseband) $\hat{y}_k$ in two steps.  First,  $\tilde{x}^Q_k[n]$ is up-sampled (interpolated) with zeros (including replacing masked symbols with zeros) to generate sequence $u_k[n]$ that has the same data rate as that of $y_k[n]$.  The interpolated sequence $u_k[n]$ is passed through a subband interpolation  filter $\Hc_k^{\dagger}$ with impulse response $\hat{h}_k[n]$ to produce an estimate of the baseband representation of the $k$th harmonic signal $\hat{y}_k[n]$.  The subband  interpolation filter may be chosen as the matched-filter $\hat{h}_k[n]=h_k[-n]$ to maximize the signal-to-noise ratio.  Other implementations, such as windowed low-pass filters, can also be used.  The decompression of the interharmonic signal directly follows the compression algorithm used at the encoder.


The final decompression step takes the subband signals $\hat{y}_k[n]$  produce an estimate of  the original direct sampled $x[n]$ of $x(t)$ in the encoder:
\begin{equation}
    \hat{x}[n]=\sqrt{2} {\rm Re} \Bigg(\sum_{k=1}^K \hat{y}_k[n]e^{j k \omega_0 n} \Bigg) + \hat{y}_e[n].
\end{equation}





==> Encode.tex <==

%
%
%\begin{center}
%\begin{figure*}[b]
%\begin{psfrags}
%\psfrag{T0}[c]{$t=nT_s$}
%\psfrag{x}[c]{ $\hat{x}[n]$}
%\psfrag{R}[c]{ ${\rm Re}$}
%\psfrag{xn}[c]{ $x[n]$}
%\psfrag{e}[l]{$e^{j\omega_0n}$}
%\psfrag{e1}[c]{$e^{j2\omega_0n}$}
%\psfrag{e2}[c]{ $e^{j3\omega_0n}$}
%\psfrag{K0}[c]{$\uparrow S_0$}
%\psfrag{K1}[c]{ $\uparrow S_1$}
%\psfrag{K2}[c]{ $\uparrow S_2$}
%\psfrag{A0}[c]{ $\hat{h}_0[n]$}
%\psfrag{A1}[c]{$\hat{h}_1[n]$}
%\psfrag{A2}[c]{$\hat{h}_2[n]$}
%\psfrag{Ae}[c]{ $\Kc_e^{\dagger}$}
%\psfrag{D0}[c]{ $$}
%\psfrag{D1}[c]{$\Dc_1$}
%\psfrag{D2}[c]{ $\Dc_2$}
%\psfrag{D3}[c]{$\Dc_3$}
%\psfrag{Q0}[c]{$\Qc_0$}
%\psfrag{Q1}[c]{ $\Qc_1$}
%\psfrag{Q2}[c]{ $\Qc_2$}
%\psfrag{Q3}[c]{ $\Qc_3$}
%\psfrag{y1}[c]{ $x^Q_0$}
%\psfrag{y2}[c]{ $x^Q_1$}
%\psfrag{y3}[c]{ $x^Q_2$}
%\psfrag{ye}[c]{ $x^Q_e$}
%\psfrag{z}[c]{ $b$}
%\psfrag{z1}[c]{ $z_0$}
%\psfrag{z2}[c]{ $z_1$}
%\psfrag{z3}[c]{ $z_2$}
%\psfrag{g1}[c]{ $\hat{y}_0[n]$}
%\psfrag{g2}[c]{ $\hat{y}_1[n]$}
%\psfrag{g3}[c]{ $\hat{y}_2[n]$}
%\psfrag{ge}[c]{ $\hat{y}_e[n]$}
%\centerline{\scalefig{0.7}\epsfbox{figs/Schematic_Decode1.eps}}
%\end{psfrags}
%\caption{A three-subband ASBC decoder.  Time indices of internal signals are obmitted with $y_i$ standing for $y[n]$.}
%\label{fig:decode}
%\end{figure*}
%\end{center}




As illustrated in Fig.~\ref{fig:encode}, an ASBC encoder  partitions the signal spectrum into a set of frequency bands,  adaptively masks inactive bands,  and encodes  the unmasked bands in parallel.    These individual components are explained below.

\vspace{-0.5em}
 \subsection{Subband decomposition} From the output of the sensor transformer, the continuous-time measurement signal $x(t)$ is sampled at $F_s$ Hz.  The discrete-time signal $x[n]$ is frequency down-shifted and passed through a  filterbank $\Hc=(\Hc_e,\Hc_1,\cdots, \Hc_K)$ that
 extracts the subband signal $x_k[n]$ in its baseband represention $y_k[n]$.  Specifically, the  output of the $k$th subband filter is a complex time series
\begin{equation}
    y_k[n] = (x[n]e^{-j k\omega_0 n}) \circledast h_k[n],~~\omega_0 := \frac{2\pi F_0}{F_s}
\end{equation}

where $\circledast$ is the convolution operator.  Ideally, the filter for the $k$th subband is a low-pass filter with bandwidth $W_k/2$, whose output $y_k[n]$ is the baseband representation of the $k$th harmonic signal $x_k[n]$.

The interharmonic distortion $y_e[n]$  whose spectrum corresponds to the grey area of power spectrum in Fig.~\ref{fig:Xf} can be  extracted  by
\begin{equation}
    y_e[n] = x[n] - \sqrt{2}{\rm Re}\bigg(\sum_{k=1}^K y_k[n]e^{jk\omega_0n})\bigg).
\end{equation}

In absence of high order and interharmonics, $x(t) = x_1(t)$ in (\ref{eq:model}), and only $y_1[n]$ is non-zero.


\begin{center}
\begin{figure*}[t]
\begin{psfrags}
\psfrag{T0}[c]{$t=nT_s$}
\psfrag{x}[c]{ $\hat{x}[n]$}
\psfrag{R}[c]{ ${\rm \sqrt{2}Re}$}
\psfrag{xn}[c]{ $x[n]$}
\psfrag{e}[l]{$e^{j\omega_0n}$}
\psfrag{e1}[c]{$e^{j2\omega_0n}$}
\psfrag{e2}[c]{ $e^{j3\omega_0n}$}
\psfrag{K0}[c]{$\uparrow S_1$}
\psfrag{K1}[c]{ $\uparrow S_2$}
\psfrag{K2}[c]{ $\uparrow S_3$}
\psfrag{A0}[c]{ $\Hc_1^\dagger$}
\psfrag{A1}[c]{$\Hc_2^\dagger$}
\psfrag{A2}[c]{$\Hc_3^\dagger$}
\psfrag{Ae}[c]{ $\Kc_e^{\dagger}$}
\psfrag{D0}[c]{ $$}
\psfrag{D1}[c]{$\Dc_1$}
\psfrag{D2}[c]{ $\Dc_2$}
\psfrag{D3}[c]{$\Dc_3$}
\psfrag{Q0}[c]{$\Qc_0$}
\psfrag{Q1}[c]{ $\Qc_1$}
\psfrag{Q2}[c]{ $\Qc_2$}
\psfrag{Q3}[c]{ $\Qc_3$}
\psfrag{y1}[c]{ $\tilde{x}^Q_1$}
\psfrag{y2}[c]{ $\tilde{x}^Q_2$}
\psfrag{y3}[c]{ $\tilde{x}^Q_3$}
\psfrag{ye}[c]{ $\tilde{x}^Q_e$}
\psfrag{z}[r]{ $b$ (bit stream)}
\psfrag{z1}[c]{ $u_0$}
\psfrag{z2}[c]{ $u_1$}
\psfrag{z3}[c]{ $u_2$}
\psfrag{g1}[c]{ $\hat{y}_1[n]$}
\psfrag{g2}[c]{ $\hat{y}_2[n]$}
\psfrag{g3}[c]{ $\hat{y}_3[n]$}
\psfrag{ge}[c]{ $\hat{y}_e[n]$}
\centerline{\scalefig{0.7}\epsfbox{figs/Schematic_Decode1.eps}}
\end{psfrags}
\caption{A three-subband ASBC decoder.  Time indices of internal signals $(x_i^Q, u_i)$ are omitted.}
\label{fig:decode}
\end{figure*}
\end{center}


\vspace{-0.5em}
\subsection{Activity detection}  Except $y_1[n]$  from the output of subband filter $\Hc_1$ corresponding to the subband associated with the system frequency $F_0$,  the outputs from the rest of subband filters are passed thorough activity detectors $(\Dc_e, \Dc_k)$  to determine the level of compression required, ranging from  transmitting  at the subband Nyquist rate to full compression that eliminates the transmission of $y_k[n]$.

The activity detection is performed on  blocks of samples. The detector $\Dc_k$  takes a block of samples and outputs an indicator $w_k=1$  for the block  if the subband $k$ is active  and $w_k=0$ otherwise.  The detector for inter-harmonic subband does the same way.   A standard implementation of the activity detector is the energy detector.  More sophisticated techniques such as quickest detection or machine-learning based detection can also be used.

%Detector $\Dc_k$ can be implemented by an energy detector on a block-by-block basis.  For a block of $M_k$ data points starting at $n-M_k+1$  and ending at $n$, let the empirical power level be
%\[
%\hat{p}_k[n] =\left\{\begin{array}{ll}
% \frac{1}{M_k}\sum_{m=0}^{M_k-1} |y_k[n-m]|^2, &~n\equiv 0 (\mbox{mod}~M_k)\\
% \sharp & \mbox{otherwise}
%\end{array}\right.,\]
%where $\sharp$ stands for ``no-value'' that is to be ignored downstream.  Detector $\Dc_k$ compares $\hat{p}_k[n]$ with a threshold $\tau$ and produces a masking function for the data block
%\bea
%z_k[n] &=& \left\{\begin{array}{ll}
%1 & \mbox{if $\hat{p}_k[n] \ge  \tau_k $, $n\equiv 0~(\mbox{mod}~M_k)$}\\
%0 & \mbox{if $\hat{p}_k[n] <  \tau_k $ and $n\equiv 0~(\mbox{mod}~M_k)$}\\
%\end{array}\right.\nn\\
%z_k[n-i] &=& z_k[n]~\mbox{for $n\equiv 0 (\mbox{mod}~M_k), 0\le i <M_k$}.\nn
%\eea
%The threshold $\tau_k$ is chosen to control the false positive rate when there is substantial energy in the $k$th harmonic while the detector $\Dc_k$ declares otherwise.


\vspace{-0.5em}
\subsection{Subband compression} The compression of the harmonic subband $k$ is achieved by down-sampling of $y_k[n]$ by $S_k$ fold.  By the (passband) Nyquist sampling theorem, if the $k$th subband has passband bandwidth of $W_k$, then the signal in the $k$th subband can be perfectly reconstructed by sampling $x_k(t)$ at frequency of $W_k$ (Hz).  Given that $x(t)$ is sampled at $F_s$ (Hz), the rate of down-sampling  $S_k$ is given by
\begin{equation}
    S_k =\Bigg\lceil \frac{F_s}{W_k} \Bigg\rceil.
\end{equation}
 If  subband $k$ is active, the down-sampler gives the compressed data sequence
\beq
\tilde{x}_k[n]=\left\{\begin{array}{ll}
y_k[nS_k], & ~\mbox{$w_k[n]=1$,}\\
\sharp, & \mbox{otherwise,}\\
\end{array}\right.
\eeq
where  $\sharp$ is a masking symbol indicating that the data  sample needs not be encoded and transmitted.  The data rate associated with $\tilde{x}_k[n]$ is at most $1/S_k$ of that of $y_k[n]$.

The interharmonic band is expected to be active infrequently. When an interharmonic signal needs to  be transmitted to the control center, an FFT-based (\eg FFT-$(k,L)$  described in Sec.~\ref{sec:FFT}) or wavelet based compression scheme can be used.
See references in \cite{Tcheou&etal:14TSG}.

\vspace{-0.5em}
\subsection{Quantization and multiplexing}   The down-sampled data streams are quantized by  quantizer $(\Qc_e,\Qc_k)$  that maps subband stream $\tilde{x}_k[n]$ into a bit-stream  $\tilde{x}^Q_k$ of $R_k$ bits/sample. A scaler quantizer such as pulse-code modulation (PCM)
quantizes individual sample of $\tilde{x}_k$ into $R_k$ bits of $\tilde{x}^Q_k$, whereas a vector quantizer such as code excited linear prediction (CLEP) or K-mean clustering takes a block of $M$ samples of and quantizes them into a block of  $MR_k$ bits of $\tilde{x}_k^Q$.   The bit-streams from subbands are multiplexed into a single bit-stream $b$ to be delivered to the receiver.
Also communicated the length of inactivity masks  for each block that is not transmitted due to inactivity.




==> Encode_v1.tex <==

%
%
%\begin{center}
%\begin{figure*}[b]
%\begin{psfrags}
%\psfrag{T0}[c]{$t=nT_s$}
%\psfrag{x}[c]{ $\hat{x}[n]$}
%\psfrag{R}[c]{ ${\rm Re}$}
%\psfrag{xn}[c]{ $x[n]$}
%\psfrag{e}[l]{$e^{j\omega_0n}$}
%\psfrag{e1}[c]{$e^{j2\omega_0n}$}
%\psfrag{e2}[c]{ $e^{j3\omega_0n}$}
%\psfrag{K0}[c]{$\uparrow S_0$}
%\psfrag{K1}[c]{ $\uparrow S_1$}
%\psfrag{K2}[c]{ $\uparrow S_2$}
%\psfrag{A0}[c]{ $\hat{h}_0[n]$}
%\psfrag{A1}[c]{$\hat{h}_1[n]$}
%\psfrag{A2}[c]{$\hat{h}_2[n]$}
%\psfrag{Ae}[c]{ $\Kc_e^{\dagger}$}
%\psfrag{D0}[c]{ $$}
%\psfrag{D1}[c]{$\Dc_1$}
%\psfrag{D2}[c]{ $\Dc_2$}
%\psfrag{D3}[c]{$\Dc_3$}
%\psfrag{Q0}[c]{$\Qc_0$}
%\psfrag{Q1}[c]{ $\Qc_1$}
%\psfrag{Q2}[c]{ $\Qc_2$}
%\psfrag{Q3}[c]{ $\Qc_3$}
%\psfrag{y1}[c]{ $x^Q_0$}
%\psfrag{y2}[c]{ $x^Q_1$}
%\psfrag{y3}[c]{ $x^Q_2$}
%\psfrag{ye}[c]{ $x^Q_e$}
%\psfrag{z}[c]{ $b$}
%\psfrag{z1}[c]{ $z_0$}
%\psfrag{z2}[c]{ $z_1$}
%\psfrag{z3}[c]{ $z_2$}
%\psfrag{g1}[c]{ $\hat{y}_0[n]$}
%\psfrag{g2}[c]{ $\hat{y}_1[n]$}
%\psfrag{g3}[c]{ $\hat{y}_2[n]$}
%\psfrag{ge}[c]{ $\hat{y}_e[n]$}
%\centerline{\scalefig{0.7}\epsfbox{figs/Schematic_Decode1.eps}}
%\end{psfrags}
%\caption{A three-subband ASBC decoder.  Time indices of internal signals are obmitted with $y_i$ standing for $y[n]$.}
%\label{fig:decode}
%\end{figure*}
%\end{center}




 As part of  the remote terminal unit, the ASBC encoder  partitions the signal spectrum into a set of frequency bands.  It  adaptively masks inactive bands and encodes  the unmasked bands in parallel.  Fig.~\ref{fig:encode} illustrates the schematic of the ASBC encoder.   The functionalities of individual components are explained below.

\vspace{-0.5em}
 \subsection{Subband decomposition} From the output of the sensor transformer, the continuous-time measurement signal $x(t)$ is sampled at $F_s$ Hz.  The discrete-time signal $x[n]$ is frequency down-shifted and passed through a  filterbank $\Hc=(\Hc_e,\Hc_1,\cdots, \Hc_K)$ that
 extracts the subband signal $x_k[n]$ in its baseband represention $y_k[n]$.  Specifically, the  output of the $k$th subband filter is a complex time series
\begin{equation}
    y_k[n] = (x[n]e^{-j k\omega_0 n}) \circledast h_k[n],~~\omega_0 := \frac{2\pi F_0}{F_s}
\end{equation}

where $\circledast$ is the convolution operator.  Ideally, the filter for the $k$th subband is a low-pass filter with bandwidth $W_k/2$, whose output $y_k[n]$ is the baseband representation of the $k$th harmonic signal $x_k[n]$.

The interharmonic distortion $y_e[n]$  whose spectrum corresponds to the grey area of power spectrum in Fig.~\ref{fig:Xf} can be  extracted  by
\begin{equation}
    y_e[n] = x[n] - \sqrt{2}{\rm Re}\bigg(\sum_{k=1}^K y_k[n]e^{jk\omega_0n})\bigg).
\end{equation}

In absence of high order and interharmonics, $x(t) = x_1(t)$ in (\ref{eq:model}), and only $y_1[n]$ is non-zero.



\vspace{-0.5em}
\subsection{Activity detection}  Except $y_1[n]$  from the output of subband filter $\Hc_1$ corresponding to the subband associated with the system frequency $F_0$,  the outputs from the rest of subband filters are passed thorough activity detectors $(\Dc_e, \Dc_k)$  to determine the level of compression required, ranging from  transmitting  at the subband Nyquist rate to full compression that eliminates the transmission of $y_k[n]$.

The activity detection is performed on  blocks of samples. The detector $\Dc_k$  takes a block of samples and outputs an indicator $w_k=1$  for the block  if the subband $k$ is active  and $w_k=0$ otherwise.  The detector for inter-harmonic subband does the same way.   A standard implementation of the activity detector is the energy detector.  More sophisticated techniques such as quickest detection or machine-learning based detection can also be used.

%Detector $\Dc_k$ can be implemented by an energy detector on a block-by-block basis.  For a block of $M_k$ data points starting at $n-M_k+1$  and ending at $n$, let the empirical power level be
%\[
%\hat{p}_k[n] =\left\{\begin{array}{ll}
% \frac{1}{M_k}\sum_{m=0}^{M_k-1} |y_k[n-m]|^2, &~n\equiv 0 (\mbox{mod}~M_k)\\
% \sharp & \mbox{otherwise}
%\end{array}\right.,\]
%where $\sharp$ stands for ``no-value'' that is to be ignored downstream.  Detector $\Dc_k$ compares $\hat{p}_k[n]$ with a threshold $\tau$ and produces a masking function for the data block
%\bea
%z_k[n] &=& \left\{\begin{array}{ll}
%1 & \mbox{if $\hat{p}_k[n] \ge  \tau_k $, $n\equiv 0~(\mbox{mod}~M_k)$}\\
%0 & \mbox{if $\hat{p}_k[n] <  \tau_k $ and $n\equiv 0~(\mbox{mod}~M_k)$}\\
%\end{array}\right.\nn\\
%z_k[n-i] &=& z_k[n]~\mbox{for $n\equiv 0 (\mbox{mod}~M_k), 0\le i <M_k$}.\nn
%\eea
%The threshold $\tau_k$ is chosen to control the false positive rate when there is substantial energy in the $k$th harmonic while the detector $\Dc_k$ declares otherwise.


\vspace{-0.5em}
\subsection{Subband compression} The compression of the harmonic subband $k$ is achieved by down-sampling of $y_k[n]$ by $S_k$ fold.  By the (passband) Nyquist sampling theorem, if the $k$th subband has passband bandwidth of $W_k$, then the signal in the $k$th subband can be perfectly reconstructed by sampling $x_k(t)$ at frequency of $W_k$ (Hz).  Given that $x(t)$ is sampled at $F_s$ (Hz), the rate of down-sampling  $S_k$ is given by
\begin{equation}
    S_k =\Bigg\lceil \frac{F_s}{W_k} \Bigg\rceil.
\end{equation}
 If  subband $k$ is active, the down-sampler gives the compressed data sequence
\beq
\tilde{x}_k[n]=\left\{\begin{array}{ll}
y_k[nS_k], & ~\mbox{$w_k[n]=1$,}\\
\sharp, & \mbox{otherwise,}\\
\end{array}\right.
\eeq
where  $\sharp$ is a masking symbol indicating that the data  sample needs not be encoded and transmitted.  The data rate associated with $\tilde{x}_k[n]$ is at most $1/S_k$ of that of $y_k[n]$.

The interharmonic band is expected to be active infrequently. When an interharmonic signal needs to  be transmitted to the control center, an FFT-based (\eg FFT-$(k,L)$  described in Sec.~\ref{sec:FFT}) or wavelet based compression scheme can be used.
See references in \cite{Tcheou&etal:14TSG}.

\vspace{-0.5em}
\subsection{Quantization and multiplexing}   The down-sampled data streams are quantized by  quantizer $(\Qc_e,\Qc_k)$  that maps subband stream $\tilde{x}_k[n]$ into a bit-stream  $\tilde{x}^Q_k$ of $R_k$ bits/sample. A scaler quantizer such as pulse-code modulation (PCM)
quantizes individual sample of $\tilde{x}_k$ into $R_k$ bits of $\tilde{x}^Q_k$, whereas a vector quantizer such as code excited linear prediction (CLEP) or K-mean clustering takes a block of $M$ samples of and quantizes them into a block of  $MR_k$ bits of $\tilde{x}_k^Q$.   The bit-streams from subbands are multiplexed into a single bit-stream $b$ to be delivered to the receiver.
Also communicated the length of inactivity masks  for each block that is not transmitted due to inactivity.
\begin{center}
\begin{figure*}[t]
\begin{psfrags}
\psfrag{T0}[c]{$t=nT_s$}
\psfrag{x}[c]{ $\hat{x}[n]$}
\psfrag{R}[c]{ ${\rm \sqrt{2}Re}$}
\psfrag{xn}[c]{ $x[n]$}
\psfrag{e}[l]{$e^{j\omega_0n}$}
\psfrag{e1}[c]{$e^{j2\omega_0n}$}
\psfrag{e2}[c]{ $e^{j3\omega_0n}$}
\psfrag{K0}[c]{$\uparrow S_1$}
\psfrag{K1}[c]{ $\uparrow S_2$}
\psfrag{K2}[c]{ $\uparrow S_3$}
\psfrag{A0}[c]{ $\Hc_1^\dagger$}
\psfrag{A1}[c]{$\Hc_2^\dagger$}
\psfrag{A2}[c]{$\Hc_3^\dagger$}
\psfrag{Ae}[c]{ $\Kc_e^{\dagger}$}
\psfrag{D0}[c]{ $$}
\psfrag{D1}[c]{$\Dc_1$}
\psfrag{D2}[c]{ $\Dc_2$}
\psfrag{D3}[c]{$\Dc_3$}
\psfrag{Q0}[c]{$\Qc_0$}
\psfrag{Q1}[c]{ $\Qc_1$}
\psfrag{Q2}[c]{ $\Qc_2$}
\psfrag{Q3}[c]{ $\Qc_3$}
\psfrag{y1}[c]{ $\tilde{x}^Q_1$}
\psfrag{y2}[c]{ $\tilde{x}^Q_2$}
\psfrag{y3}[c]{ $\tilde{x}^Q_3$}
\psfrag{ye}[c]{ $\tilde{x}^Q_e$}
\psfrag{z}[r]{ $b$ (bit stream)}
\psfrag{z1}[c]{ $u_0$}
\psfrag{z2}[c]{ $u_1$}
\psfrag{z3}[c]{ $u_2$}
\psfrag{g1}[c]{ $\hat{y}_1[n]$}
\psfrag{g2}[c]{ $\hat{y}_2[n]$}
\psfrag{g3}[c]{ $\hat{y}_3[n]$}
\psfrag{ge}[c]{ $\hat{y}_e[n]$}
\centerline{\scalefig{0.7}\epsfbox{figs/Schematic_Decode1.eps}}
\end{psfrags}
\caption{A three-subband ASBC decoder.  Time indices of internal signals $(x_i^Q, u_i)$ are omitted.}
\label{fig:decode}
\end{figure*}
\end{center}




==> Intro_final.tex <==
We consider the problem of pricing multi-interval look-ahead economic dispatch when generators are ramp-constrained and demand forecasts inaccurate.   This work is motivated by  recent discussions among system operators on the need for ramping products in response to the ``duck-curve'' effect of renewable integrations \cite{Xie&Luo&Obadina:11PESGM,Peng&Chatterjee:13FERC,CAISO_FRP:15,Mickey:15,Parker:15,%
Schiro:17}.   A well-designed multi-interval look-ahead dispatch that anticipates trends of future demand can minimize the use of more expensive ramp resources. %\cite{XIA&Elaiw:10EPSR}.

A standard implementation of a look-ahead dispatch is the so-called {\em rolling-window dispatch}, where the operator optimizes the dispatch over a few scheduling intervals into the future based on load forecasts.  The dispatch for the immediate scheduling interval ({\it a.k.a. the binding interval}) is implemented while the dispatch for the subsequent intervals serves as an advisory signal and is updated sequentially.  A common practice to price the rolling-window dispatch is the rolling-window version of the multi-interval locational marginal pricing (LMP).


LMP is a uniform pricing mechanism across generators and demands at the same location in the same scheduling interval. For the single-interval pricing problem, LMP has remarkable properties.  LMP supports an efficient market equilibrium such that a profit-maximizing generator has no incentive to deviate from the central dispatch.   For a competitive market with a large number of generators, a price-taking generator has the incentive to bid truthfully at its marginal cost of generation.    LMP also guarantees a nonnegative merchandising surplus for the system operator. As a uniform pricing scheme, LMP is transparent to all market participants, and the price can be computed easily as a by-product of the underlying economic dispatch.


Most of the attractive features of LMP are lost, unfortunately, when the  rolling-window version of LMP (R-LMP) is used and demand forecasts inaccurate.  Indeed, even if perfect forecasts are used in R-LMP,  many nice properties of LMP  are not guaranteed.  In particular, a missing-money scenario arises when a  generator is asked to hold back its generation in order to provide ramping support for the system to meet  demands in future intervals.  In doing so, the generator incurs an opportunity cost and may be paid below its  offered price to generate.   Expecting compensations in future intervals for the opportunity costs, the generator disappoints when the anticipated higher payments do not realize due to changing demand forecasts.    Examples of such scenarios are well known and also illustrated in Example 2 in Sec~\ref{sec:example}.  It turns out that such examples are not isolated instances unique to R-LMP.  As we show in  Theorem~\ref{thm:UniformPricingLOC} in Sec.~\ref{sec:incentives}, they occur under all uniform pricing schemes.

To ensure that generators are adequately compensated, the operator  provides the so-called {\em uplift payments}  to generators suffering from underpayments in an {\em out-of-the-market settlement.}    The roles of  uplifts have been discussed extensively in the literature \cite{Gribik&Hogan&Pope:07,Zhang&Luh&Litvinov&Zheng&Zhao:09PESGM,Al-Abdullah&Abdi-Khorsand&Hedman:15TPS,Zhang&Hedman:19NAPS}.   Such settlements are typically discriminative and subject to manipulation.   Examples exist that, under LMP,  a price-taking generator may have incentives to deviate from truthful-bidding to take advantage the out-of-the-market settlements.  See Appendix I.



\subsection{Related work}
Wilson discussed the issue of pricing distortion introduced by ramping in \cite{Wilson:02E}.  He pointed out that the cause of such pricing distortion is that the optimization model used in price formation is imperfect.  In the rolling-widow dispatch context, both the imperfection of demand forecasts and the limited look-ahead distort the dispatch-following incentives.  The use of out-of-the-market uplifts further distorts the truthful-bidding incentives.  The dispatch-following incentive issues in pricing multi-interval dispatch  have been widely discussed in the literature \cite{Peng&Chatterjee:13FERC,Ela&OMalley:16TPS,%
Schiro:17,Guo&Tong:18Allerton,Hua&etal:19TPS,Zhao&Zheng&Litvinov:19arxiv,Zhang&Hedman:19NAPS}, although a formal way of analyzing such issues is lacking.  The effects of the out-of-the-market uplifts on truthful-bidding incentives are not well understood.

Several marginal cost pricing schemes have been proposed for the rolling-window dispatch policies.  The flexible ramping product (FRP) \cite{CAISO_FRP:15} treats ramping as a product to be procured and priced uniformly as part of the real-time dispatch.  FRP is a two-part tariff consisting of prices of energy and ramping.  Ela and O'Malley proposed the cross-interval marginal price (CIMP) in \cite{Ela&OMalley:16TPS} defined by the sum of marginal costs with respect to the demands in the binding and the future (advisory) intervals.  Multi-settlement pricing schemes are proposed in \cite{Schiro:17FERC,Zhao&Zheng&Litvinov:19arxiv} that generalize the existing two-settlement day-ahead and real-time markets.

Deviating from marginal cost pricing are two recent proposals aimed at minimizing the out-of-the-market payments; both employ separate pricing optimizations that are different from that used in the economic dispatch.    The price-preserving multi-interval pricing (PMP), initially suggested by Hogan in \cite{Hogan:16} and formalized in \cite{Hua&etal:19TPS}, adds to the objective function the loss-of-opportunity cost for the generators for the realized prices and dispatch decisions.   In contrast, the constraint-preserving multi-interval pricing (CMP) proposed in  \cite{Hua&etal:19TPS} fixes the past dispatch decisions and penalizes ramping violations.  Both have shown improvements over the standard R-LMP policy.

 All existing pricing schemes for multi-interval economic dispatch are based on uniform pricing mechanisms.  To our best knowledge, no existing pricing policies can provide dispatch-following incentives that eliminate discriminative out-of-the-market settlements.


\subsection{Summary of results, contexts, and limitations}
The main contribution of this work is threefold.   First, we show in Theorem~\ref{thm:UniformPricingLOC} that price discrimination is  unavoidable in pricing rolling-window dispatch.  Specifically,   all uniform pricing mechanisms require some level of out-of-the-market uplifts under the rolling-window dispatch model.  While uniform pricing schemes are transparent and  non discriminative within the market clearing process, it is the  out-of-the-market uplift payments that make the overall payment scheme discriminative.

Second, we  generalize LMP to a nonuniform pricing scheme, referred to as the {\em temporal locational marginal pricing (TLMP)}.  TLMP prices the production of a generator $i$ based on its contribution to meeting the demand in interval $t$.  In doing so, TLMP encapsulates both generation and ramping-induced opportunity costs in each interval.

As shown in Proposition~\ref{prop:TLMP}, TLMP decomposes into energy and ramping prices:
\beq \label{eq:TLMP0}
\pi_{it}^{\TLMP}=\pi_{t}^{\LMP} + \mu_{it}-\mu_{i(t-1)},
\eeq
where $\pi_{t}^{\LMP} $ is the standard LMP, and the second term is the increment of the Lagrange multipliers associated with the ramping constraints in the economic dispatch optimization, from $\mu_{i(t-1)}$  in interval $(t-1)$ to $\mu_t$ in interval $t$.   The above decomposition is analogous to the energy-congestion price decomposition of LMP.  TLMP naturally reduces to LMP in the absence of binding ramping constraints.

Third, we establish several key properties that make TLMP a viable and potentially attractive alternative to standard uniform pricing schemes. A key  property of TLMP is that, under the dispatch and pricing models assumed in this paper, the rolling-window implementation of TLMP (R-TLMP) eliminates the need of out-of-the-market uplifts for the rolling-window economic dispatch under arbitrary forecast errors.  Whereas all pricing schemes are necessarily discriminative,  R-TLMP stands out as one that discriminates inside rather than outside  the market clearing process.  This property ties  real-time pricing closely to the actually realized ramping conditions.

As a generalization of LMP, TLMP extends some of the important properties of LMP to the rolling-window  multi-interval pricing setting, thanks to the property that R-TLMP is a strong equilibrium price that decouples the profit maximization problem over the entire scheduling horizon into  single-interval ones.  A significant property of TLMP (Theorem~\ref{thm:TLMPBid}) is that a price-taking profit-maximizing generator has the incentive to bid truthfully with its marginal cost of generation.   In other words, there is no need for a generator to internalize ramping-induced opportunity  costs.  Such a property, however,  does not hold for the rolling-window implementation of the multi-interval LMP.  See Appendix I.


Also significant (Proposition 3 of Part II) is that, under TLMP, the operator's merchandising surplus is the sum of congestion and ramping surplus, which has significant implications on the revenue adequacy of ISO.    We also demonstrate that, under TLMP, the generators have incentives for truthful  revelation of ramping limits, and there are incentives for the generators to improve their ramping capabilities.


Given that TLMP is discriminatory, one may question how different it is from other discriminative pricing schemes such as the  pay-as-bid (PAB) pricing.   The differences between TLMP and PAB pricing are significant; TLMP is much closer to LMP than it is to PAB.   Comparing with LMP, PAB is more vulnerable to manipulative bidding behaviors, and a market participant has little incentive to bid truthfully.   In contrast, TLMP inherits and extends (in Theorem \ref{thm:TLMPBid}) the property of LMP (under the single-interval model) that a price taker generator bids truthfully with its marginal cost.

Discriminative pricing is often criticized for its lack of  transparency, which makes it difficult for the operator to provide public pricing signals to market participants.  Because of the decomposition of TLMP into the uniform energy price (LMP)  and a discriminative ramping price in (\ref{eq:TLMP0}), the energy part of TLMP (LMP) is transparent to all participants.   The ramping price part of TLMP, like the out-of-the-market uplifts, is nontransparent and discriminative.  In this aspect, TLMP has the same level of transparency as in LMP, although the amount of the discriminative payments under TLMP and  uniform prices can be quite different.  See Part II of this paper for a numerical comparison \cite{Chen&Guo&Tong:20TPS}.

Finally, in Part II of the paper, we generalize the theory of dispatch-following incentives to more general models that include network constraints and discuss a broader set of incentive and performance issues through numerical simulations.    When comparing different pricing schemes, our results shine lights on practical tradeoffs along several dimensions:  the revenue adequacy of the ISO, consumer payments, generator profits, and price volatilities.

A few words are in order on the scope and limitations of this paper.
We do not model strategic behaviors of the generators, nor do we consider those market models that the market operator does not price ramping costs and lets the generators internalize their individual ramping costs. We discuss in Sec.~\ref{sec:discussion} some of the implications of these omissions.   We also ignore the role of unit commitment and the costs of  reserves.   In Part I,  we illustrate the properties of LMP and TLMP with a toy example.  Generalizations to systems with network constraints and more elaborate numerical examples are in Part II.

\subsection{Notations and nomenclature}
Designated symbols are listed in Table~I.
Otherwise, notations used here are standard.  We use $(x_1,\cdots,x_N)$ for a {\em column vector} and  $[x_1,\cdots,x_N]$ a {\em row vector.}    All vectors are denoted by lower-case boldface letters,  nominally as columns.   The transpose of vector $\xbf$ is denoted by $\xbf^{\tiny \intercal}$.  Matrices are boldface capital letters. Matrix $\Xbf=[x_{ij}]$  is a matrix with $x_{ij}$ as its $(i,j)$th entry.   Similar to the vector notation, matrix $\Xbf=[\xbf_1,\cdots,\xbf_N]$ has  $\xbf_i$ as its $i$th column, and matrix $\Xbf=(\xbf^{\intercal}_1,\cdots,\xbf^{\intercal}_N)$ has $\xbf_i^{\intercal}$ as its $i$th row.



{\small
\begin{table}[h]\label{tab:symbols}
\caption{\small Major symbols (in alphabetic order).}
\begin{center}
\begin{tabular}{|ll|}
\hline
${\bf 0}, {\bf 1}$: & vector of all zeros and ones.\\
$\Abf$: & a $W\times(W+1)$ matrix with $A_{ii}=-1$,\\
&$A_{i(i+1)}=1,\forall i \in \{1,...,W\}$ and zero otherwise,\\
& where $W$ is the size of the rolling window.\\\hline
% the upper bi-diagonal matrix with $-1$ as \\
% & diagonals and 1 as off diagonals.  \\\hline
$d_t$: &  the demand in interval $t$.  \\
$\dbf_t$:  &$\dbf_t=(d_t,\cdots, d_{t+W-1})$,  the demand in the \\
& look-ahead window of $W$ intervals.\\
$\dbf$: & $\dbf=(d_1,\cdots, d_T)$   the overall demand vector. \\
$\hat{d}_t, \hat{\dbf}_t$: & demand forecasts of $d_t$ and $\dbf_t$.\\\hline
$f_{it}(\cdot)$: & the bid-in cost  of generator $i$ in interval $t$. \\
$F(\cdot)$: & aggregated bid-in cost curve in $W$ or $T$ intervals.\\
$F_{-it}(\cdot)$: & aggregated bid-in cost curve excluding generation \\
& from generator $i$ in interval $t$.\\\hline
$g_{it}$: & generation/dispatch of generator $i$ in interval $t$ \\
$\gbf[t]$: & generation/dispatch vector for all generators in\\
 & interval $t$, $\gbf[t]=(g_{1t},\cdots, g_{Nt})$.\\
$\Gbf$: & generation/dispatch matrix. $\Gbf=\big[\gbf[1],\cdots,\gbf[T]\big]$.\\
$\gbf_i$: & dispatch of generator $i$ over a scheduling window, \\
& \eg $\gbf_i=(g_{i1},\cdots, g_{iW})$ or $\gbf_i=(g_{i1},\cdots, g_{iT})$. \\\hline
$\Gc_t$: & the  look-ahead dispatch policy at time $t$.\\
$\Gc^{\mbox{\tiny ED}}_t$: & the look-ahead  economic dispatch policy at time $t$.\\
$\gbf_i^{\ED}$: &  one-shot economic dispatch for generator $i$.\\
$\gbf_i^{\RED}$: & rolling-window economic dispatch for generator $i$.\\\hline
$\Hmsc_t$: & scheduling window $\Hmsc_t=\{t,\cdots, t+W-1\}$.\\
$\Hmsc$: & scheduling horizon  $\Hmsc=\{1,\cdots, T\}$.\\\hline
$\mbox{LOC}$: & lost-of-opportunity cost uplift. \\
$\mbox{MW}$: & make-whole uplift.\\\hline
$\Pc_t, \Pc^{\mbox{\tiny LMP}}_t$: & multi-interval pricing policy and LMP pricing policy.\\
$\pibf^{\LMP},\pibf^{\TLMP}$: & one-shot LMP and TLMP.\\
$\pibf^{\RLMP},\pibf^{\RTLMP}$: & rolling-window LMP/TLMP. \\\hline
$q_{it}(\cdot), \qbf_i(\cdot)$: & true cost of generation of generator $i$.\\
$T$: & total number of scheduling intervals. \\
$W$:& scheduling window size. $W\le T$.\\\hline
\end{tabular}
%\caption{\small Major symbols (in alphabetic order).}
\end{center}
\end{table}
}





==> Model.tex <==


We model  the continuous-time voltage (or current) signal $x(t)$  as the sum of $K$ harmonics $x_k(t)$ and an interharmonic component $e(t)$:

\vspace{-1em}
\begin{subequations}\label{eq:model}
\begin{align}
x(t)&=  \sum_{k=1}^K x_k(t) + e(t), \label{eq:xa}\\
x_k(t) &=  a_k(t) \cos(k\Omega_0 t + \phi_k(t)),  \label{eq:xb}
\end{align}
\end{subequations}
where $x_1(t)$ is the signal component associated with the system frequency $F_0$   (\eg $50$ or $60$ Hz),  $\Omega_0=2\pi F_0$,
$x_k(t)$ the $k$th harnomic centered around $kF_0$, and $K-1$  the total number of  higher-order harmonics\footnote{The IEEE Standard C37.118.2-2011 suggests to include higher order harmonics up to the 50th order ($K=50$).}.   Here we allow $x_1(t)$ and its harmonics $x_k(t)$ to  take the general analytical form of (\ref{eq:xb}).  The interharmonic $e(t)$   models  noise outside the harmonic subbands.



\begin{figure}[h]
\begin{psfrags}
\psfrag{w}[c]{$W_0$}
\psfrag{wa}[c]{ $W_1$}
\psfrag{wb}[c]{ $W_2$}
\psfrag{w0}[c]{ $f$}
\psfrag{w1}[c]{ $F_0$}
\psfrag{w2}[c]{ $2F_0$}
\psfrag{w3}[c]{ $3F_0$}
\psfrag{X}[c]{$|X(f)|$}
\scalefig{0.5}\epsfbox{figs/spectrumC.eps}
\end{psfrags}
\caption{\small The spectrum of $x(t)$ and its harmonics.  The grey area represents the spectrum of interharmonics.}
\label{fig:Xf}
\end{figure}


 Let $X(f), X_k(f)$ and $E(f)$  be the Fourier spectra\footnote{Here we assume the existence of Fourier transforms of all signals.}
  of $x(t)$, $x_k(t)$, and $e(t)$, respectively, as illustrated  in Fig.~\ref{fig:Xf}.   We assume that the spectrum $X_k(f)$  of the $k$th harmonic $x_k(t)$  is
centered around $kF_0$  with passband bandwidth\footnote{The {\em passband bandwidth} is defined by the width of the frequency band containing non zero frequency components.} $W_k < F_0$.   The total bandwidth of $x(t)$ is therefore $KF_0+\frac{W_K}{2}\le (K+\frac{1}{2})F_0$.





Sampled at the frequency  $F_s$ (Hz), the discrete-time signal is given by, for $n= 0, \pm 1,  \cdots$,
\begin{subequations}\label{eq:x[n]}
\begin{align}
x[n] &:= x(nT_s) =   \sum_{k=1}^K x_k[n] + e[n],  \\
x_k[n] &:=  a_k[n] \cos\bigg(k\frac{\Omega_0}{F_s} n + \phi_k[n]\bigg),
\end{align}
\end{subequations}
where $(a_k[n], \phi_k[n])$ are the sampled amplitudes and phase angles, and $e[n]$  is the interharmonic signal.
%Let $X(\omega)=\sum_n x[n] e^{-j\omega n}$ be the discrete-time Fourier transform (DTFT) of $x[n]$.


\tcb{Unlike CPOW data, PMU measurements are complex phasors and real frequency measurements that are slowly varying.  To incorporate PMU data model in the same framework, we make a slight generalization of (\ref{eq:model}) by modeling  $x(t)$  as a single subband {\em complex signal} with $\Omega_0=0$ as
\begin{equation}
    x(t)=a_0(t)e^{j\phi_0(t)}.
    \label{eq:Synchrophasor}
\end{equation}
A special form of the above is used by the IEEE C37.118.1-2011 standard for PMU dynamic compliance evaluation\footnote{The IEEE standard C37.118.1-2011 uses the model $x(t)= \frac{X_m}{\sqrt{2}}(1+k_x\cos(\omega t))\angle k_a\cos(\omega t-\pi)$ for dynamic compliance evaluation.}.  The CPOW data compression techniques developed here applies to PMU data  with little modification.}





\begin{center}
\begin{figure*}[t]
\begin{psfrags}
\psfrag{T0}[c]{\small $t=nT_s$}
\psfrag{x}[c]{  $x(t)$}
\psfrag{xn}[c]{  $x[n]$}
\psfrag{e}[c]{  $e^{-j\omega_0n}$}
\psfrag{Ke}[c]{ $\Kc_e$}
\psfrag{K0}[c]{ $\downarrow S_1$}
\psfrag{K1}[c]{ $\downarrow S_2$}
\psfrag{K2}[c]{ $\downarrow S_3$}
\psfrag{K3}[c]{ $\downarrow S_4$}
%\psfrag{Ae}[c]{  $H_e(z)$}
%\psfrag{A0}[c]{ $H_0(z)$}
%\psfrag{A1}[c]{ $H_1(z)$}
%\psfrag{A2}[c]{$H_2(z)$}
%\psfrag{A3}[c]{ $H_3(z)$}
\psfrag{Ae}[c]{  $\Hc_e$}
\psfrag{A0}[c]{ $\Hc_1$}
\psfrag{A1}[c]{ $\Hc_2$}
\psfrag{A2}[c]{$\Hc_3$}
\psfrag{D0}[c]{ $$}
\psfrag{De}[c]{  $\Dc_e$}
\psfrag{D1}[c]{  $\Dc_2$}
\psfrag{D2}[c]{  $\Dc_3$}
\psfrag{D3}[c]{  $\Dc_3$}
\psfrag{Qe}[c]{  $\Qc_e$}
\psfrag{Q0}[c]{  $\Qc_1$}
\psfrag{Q1}[c]{  $\Qc_2$}
\psfrag{Q2}[c]{  $\Qc_3$}
\psfrag{Q3}[c]{  $\Qc_3$}
\psfrag{xe}[c]{    $\tilde{x}_e$}
\psfrag{x1}[c]{    $\tilde{x}_1$}
\psfrag{x2}[c]{    $\tilde{x}_2$}
\psfrag{x3}[c]{     $\tilde{x}_3$}
\psfrag{ye}[c]{    $\tilde{x}^Q_e$}
\psfrag{y1}[c]{    $\tilde{x}^Q_1$}
\psfrag{y2}[c]{     $\tilde{x}^Q_2$}
\psfrag{y3}[c]{     $\tilde{x}^Q_3$}
\psfrag{z}[l]{     $b$ (bit stream)}
\psfrag{ze}[c]{     $y_e$}
\psfrag{z1}[c]{     $y_1$}
\psfrag{z2}[c]{  $y_2$}
\psfrag{z3}[c]{    $y_3$}
\psfrag{z4}[c]{    $y_3[n]$}
\psfrag{ge}[c]{    $(y_e, w_e)$}
\psfrag{g1}[c]{    $(y_2, w_2)$}
\psfrag{g2}[c]{   $(y_3, w_3)$}
\psfrag{g3}[c]{    $(y_3, w_3)$}
\centerline{\scalefig{0.8}\epsfbox{figs/Schematic_Encode1.eps}}
\end{psfrags}
\caption{A three-subband ASBC encoder where $h_k[n]$  is the impulse response  of the $k$th subband filter.  Time indices of  signals are obmitted with $y_i$ standing for sequence $(y_i[n])$.}
\label{fig:encode}
\end{figure*}
\end{center}



==> Model_v2.tex <==


We model  the continuous-time voltage (or current) signal $x(t)$  as the sum of $K$ harmonics $x_k(t)$ and an interharmonic component $e(t)$:

\vspace{-1em}
\begin{subequations}\label{eq:model}
\begin{align}
x(t)&=  \sum_{k=1}^K x_k(t) + e(t), \label{eq:xa}\\
x_k(t) &=  a_k(t) \cos(k\Omega_0 t + \phi_k(t)),  \label{eq:xb}
\end{align}
\end{subequations}
where $x_1(t)$ is the signal component associated with the system frequency $F_0$   (\eg $50$ or $60$ Hz),  $\Omega_0=2\pi F_0$,
$x_k(t)$ the $k$th harnomic centered around $kF_0$, and $K-1$  the total number of  higher-order harmonics\footnote{The IEEE Standard C37.118.2-2011 suggests to include higher order harmonics up to the 50th order ($K=50$).}.   Here we allow $x_1(t)$ and its harmonics $x_k(t)$ to  take the general analytical form of (\ref{eq:xb}).  The interharmonic $e(t)$   models  noise outside the harmonic subbands.



\begin{figure}[h]
\begin{psfrags}
\psfrag{w}[c]{$W_0$}
\psfrag{wa}[c]{ $W_1$}
\psfrag{wb}[c]{ $W_2$}
\psfrag{w0}[c]{ $f$}
\psfrag{w1}[c]{ $F_0$}
\psfrag{w2}[c]{ $2F_0$}
\psfrag{w3}[c]{ $3F_0$}
\psfrag{X}[c]{$|X(f)|$}
\scalefig{0.5}\epsfbox{figs/spectrumC.eps}
\end{psfrags}
\caption{\small The spectrum of $x(t)$ and its harmonics.  The grey area represents the spectrum of interharmonics.}
\label{fig:Xf}
\end{figure}


 Let $X(f), X_k(f)$ and $E(f)$  be the Fourier spectra\footnote{Here we assume the existence of Fourier transforms of all signals.}
  of $x(t)$, $x_k(t)$, and $e(t)$, respectively, as illustrated  in Fig.~\ref{fig:Xf}.   We assume that the spectrum $X_k(f)$  of the $k$th harmonic $x_k(t)$  is
centered around $kF_0$  with passband bandwidth\footnote{The {\em passband bandwidth} is defined by the width of the frequency band containing non zero frequency components.} $W_k < F_0$.   The total bandwidth of $x(t)$ is therefore $KF_0+\frac{W_K}{2}\le (K+\frac{1}{2})F_0$.





Sampled at the frequency  $F_s$ (Hz), the discrete-time signal is given by, for $n= 0, \pm 1,  \cdots$,
\begin{subequations}\label{eq:x[n]}
\begin{align}
x[n] &:= x(nT_s) =   \sum_{k=1}^K x_k[n] + e[n],  \\
x_k[n] &:=  a_k[n] \cos\bigg(k\frac{\Omega_0}{F_s} n + \phi_k[n]\bigg),
\end{align}
\end{subequations}
where $(a_k[n], \phi_k[n])$ are the sampled amplitudes and phase angles, and $e[n]$  is the interharmonic signal.
%Let $X(\omega)=\sum_n x[n] e^{-j\omega n}$ be the discrete-time Fourier transform (DTFT) of $x[n]$.


Unlike CPOW data, PMU measurements are complex phasors and real frequency measurements that are slowly varying.  To incorporate PMU data model in the same framework, we make a slight generalization of (\ref{eq:model}) by modeling  $x(t)$  as a single subband {\em complex signal} with $\Omega_0=0$ as
\begin{equation}
    x(t)=a_0(t)e^{j\phi_0(t)}.
    \label{eq:Synchrophasor}
\end{equation}
A special form of the above is used by the IEEE C37.118.1-2011 standard for PMU dynamic compliance evaluation\footnote{The IEEE standard C37.118.1-2011 uses the model $x(t)= \frac{X_m}{\sqrt{2}}(1+k_x\cos(\omega t))\angle k_a\cos(\omega t-\pi)$ for dynamic compliance evaluation.}.  The CPOW data compression techniques developed here applies to PMU data  with little modification.





\begin{center}
\begin{figure*}[t]
\begin{psfrags}
\psfrag{T0}[c]{\small $t=nT_s$}
\psfrag{x}[c]{  $x(t)$}
\psfrag{xn}[c]{  $x[n]$}
\psfrag{e}[c]{  $e^{-j\omega_0n}$}
\psfrag{Ke}[c]{ $\Kc_e$}
\psfrag{K0}[c]{ $\downarrow S_1$}
\psfrag{K1}[c]{ $\downarrow S_2$}
\psfrag{K2}[c]{ $\downarrow S_3$}
\psfrag{K3}[c]{ $\downarrow S_4$}
%\psfrag{Ae}[c]{  $H_e(z)$}
%\psfrag{A0}[c]{ $H_0(z)$}
%\psfrag{A1}[c]{ $H_1(z)$}
%\psfrag{A2}[c]{$H_2(z)$}
%\psfrag{A3}[c]{ $H_3(z)$}
\psfrag{Ae}[c]{  $\Hc_e$}
\psfrag{A0}[c]{ $\Hc_1$}
\psfrag{A1}[c]{ $\Hc_2$}
\psfrag{A2}[c]{$\Hc_3$}
\psfrag{D0}[c]{ $$}
\psfrag{De}[c]{  $\Dc_e$}
\psfrag{D1}[c]{  $\Dc_2$}
\psfrag{D2}[c]{  $\Dc_3$}
\psfrag{D3}[c]{  $\Dc_3$}
\psfrag{Qe}[c]{  $\Qc_e$}
\psfrag{Q0}[c]{  $\Qc_1$}
\psfrag{Q1}[c]{  $\Qc_2$}
\psfrag{Q2}[c]{  $\Qc_3$}
\psfrag{Q3}[c]{  $\Qc_3$}
\psfrag{xe}[c]{    $\tilde{x}_e$}
\psfrag{x1}[c]{    $\tilde{x}_1$}
\psfrag{x2}[c]{    $\tilde{x}_2$}
\psfrag{x3}[c]{     $\tilde{x}_3$}
\psfrag{ye}[c]{    $\tilde{x}^Q_e$}
\psfrag{y1}[c]{    $\tilde{x}^Q_1$}
\psfrag{y2}[c]{     $\tilde{x}^Q_2$}
\psfrag{y3}[c]{     $\tilde{x}^Q_3$}
\psfrag{z}[l]{     $b$ (bit stream)}
\psfrag{ze}[c]{     $y_e$}
\psfrag{z1}[c]{     $y_1$}
\psfrag{z2}[c]{  $y_2$}
\psfrag{z3}[c]{    $y_3$}
\psfrag{z4}[c]{    $y_3[n]$}
\psfrag{ge}[c]{    $(y_e, w_e)$}
\psfrag{g1}[c]{    $(y_2, w_2)$}
\psfrag{g2}[c]{   $(y_3, w_3)$}
\psfrag{g3}[c]{    $(y_3, w_3)$}
\centerline{\scalefig{0.8}\epsfbox{figs/Schematic_Encode1.eps}}
\end{psfrags}
\caption{A three-subband ASBC encoder where $h_k[n]$  is the impulse response  of the $k$th subband filter.  Time indices of  signals are obmitted with $y_i$ standing for sequence $(y_i[n])$.}
\label{fig:encode}
\end{figure*}
\end{center}



==> Performance.tex <==


The standard measure of lossy compression is the rate-distortion curve that highlights the tradeoff between the level of compression and the accuracy of the reconstruction.  A well designed compression scheme has a monotonic rate-distortion curve: the higher the rate of the compressed signal, the lower the compression ratio,  the lower the distortion.

 In this paper, we adopt the compression ratio and  the normalized mean-squared error to characterize the rate-distortion characteristics.
Given a compression scheme $\chi$,  its {\em compression ratio\footnote{The theoretical compression ratio is defined by excluding protocol overhead that  has sublinear growth with the data length.}} defined by
\beq \label{eq:CR}
\eta^{\chi} =  \frac{R^{\text{uc}}}{R^{\chi}},
 \eeq
where $R^{\text{uc}}$  is the data rate (bits/sec) of the uncompressed signal and  $R^{\chi}$ the rate of the compressed stream.

Let $x[n]$ be the original (uncompressed) signal and $\hat{x}^{\chi}[n]$ the reconstructed signal at the decoder.
The {\em normalized mean-squared error (NMSE)} in (dB) is defined  by
\bea
    \Ec^{\chi} &=&10\log_{10} \frac{\sum_{n=1}^{N}|x[n]-\hat{x}^{\chi}[n]|^2}{\sum_{n=1}^{N}x^2[n]}~~(\mbox{dB})\nn\\
    &\rightarrow& 10\log_{10} \frac{\mbbE(|x[n]-\hat{x}^{\chi}[n]|^2)}{\mbbE(|x[n]|^2)} =(\text{\rm SNR}^{\chi})^{-1}    \label{eq:NMSE}
\eea
where $N$ is the length of the data sequence, and the mean-square convergence of (\ref{eq:NMSE}) assumes regularity conditions.
Note that  $\frac{1}{\Ec^{\chi}}$  has the interpretation to be the  signal-to-reconstruction noise ratio (SNR).



For the application at hand, the data rate of the uncompressed data stream can be measured by
\begin{equation}
    R^{\text{uc}}=F_sR_Q~ \mbox{(bits/sec)}
\end{equation}
where $F_s$ represents the sampling frequency of the measured signal $x(t)$ and $R_Q$  the rate of quantization (bits/sample).
The distortion of the uncompressed scheme comes only from quantization error.  With  $R_Q$ bits  PCM quantization,  the NMSE is approximately  by  
\begin{equation}
    \Ec^{\text{uc}} \approx  -6R_Q  + 1.25~~({\rm dB}).
\end{equation}


\subsection{Rate-distortion measure of  ASBC: $(\eta^{\text{ASBC}},\Ec^{\text{ASBC}})$}
We provide a characterization of the compression ratio $\eta^{\text{ASBC}}$ and the NMSE of the reconstruction $\Ec^{\text{ASBC}}$.

The data rate of the  compressed data stream by ASBC is
\begin{equation}
    R^{\text{ASBC}}= \sum_{k=1}^{K} p_k\frac{F_s}{S_k}R_k + p_e F_s R_e~ \mbox{(bits/sec)},
\end{equation}
where $F_s$   is the sampling frequency of the uncompressed data, $p_k$ the probability of $k$th subband being active, $R_k$  the rate (bits/sample) of the quantization  in  the $k$th subband, $S_k$ the down-sampling rate of $k$th subband, $p_e$ the probability that the interharmonic subband is active, and $R_e$ the rate of quantization of the  interharmonic subband.     The compression ratio of ASBC is given by
\begin{equation}
        \eta^{\text{ASBC}} = \frac{R^{\text{uc}}}{R^{\text{ASBC}}}=\left(\sum_{k=1}^{K}p_k\frac{R_k}{R_QS_k} + p_e \frac{R_e}{R_Q}\right)^{-1}.
    \label{CompressionRate}
\end{equation}
If we ignore quantization, ASBC gains via adaptively down-sampling of subband signals based on subband activity.  As an example, for the 6kHz sampling of the original signal and a harmonic subband of 6Hz bandwidth, ASBC achieves  the compression ratio $1000:1$ for that subband.


The NMSE measure $\Ec^{\text{ASBC}}$ of ASBC depends on how accurately ASBC can detect the activities of harmonic and interharmonic subbands. Assuming all harmonic subbands are active and there is no interharmonics, \ie $p_e=0$, we have $\Ec^{\text{ASBC}} \approx \Ec^{\text{uc}}$ because ASBC achieves perfect reconstruction of each harmonic signals by the Nyquist sampling theorem.  In practice, $\Ec^{\text{ASBC}} > \Ec^{\text{uc}}$ when  false negative detection occurs or when there is interharmonic signal.


\subsection{Rate-distortion measure of FFT-$(k,L)$ : $(\eta^{\text{FFT}},\Ec^{\text{FFT}})$} \label{sec:FFT}
A benchmark compression scheme is based on the fast Fourier transform (FFT), herein referred to  as FFT-$(k,L)$.  It  takes a block of $L$ data samples, computes the FFT coefficients, and keeps only the $k$ largest coefficients {$X_{j}^{(1)},\cdots,X_{j}^{(k)} $} (corresponding to the positive frequencies in the $j^{th}$ block) and masks the rest.

The compression ratio of FFT-$(k,L)$  is given by
\begin{equation}
    \eta^{\text{FFT-$(k,L)$}} = \frac{L}{k},
\end{equation}
where we ignore the $\log_2 L$ bits needed to encode the frequency locations.
The NMSE of FFT-$(k,L)$  is given by
\begin{equation}
    \Ec^{\text{FFT-$(k,L)$}} = 10\log\bigg( 1-\frac{\sum_{j=1}^{N/L}\sum_{i=1}^{k} |{X_{j}^{(i)}}|^2}{\sum_{i=1}^N |x[i]|^2}\bigg).
\end{equation}



==> Performance_v1.tex <==


The standard measure of lossy compression is the rate-distortion curve that highlights the tradeoff between the level of compression and the accuracy of the reconstruction.  In general, a well designed compression scheme should have a monotonic rate-distortion curve: the higher the rate of the compressed signal, the lower the compression ratio,  the lower the distortion.

 In this paper, we adopt the compression ratio and  the normalized mean-squared error to characterize the rate-distortion characteristics.
Given a compression scheme $\chi$,  its {\em compression ratio\footnote{The theoretical compression ratio is defined by excluding protocol overhead that  has sublinear growth with the data length.}} defined by
\beq \label{eq:CR}
\eta^{\chi} =  \frac{R^{\text{uc}}}{R^{\chi}},
 \eeq
where $R^{\text{uc}}$  is the data rate (bits/sec) of the uncompressed signal and  $R^{\chi}$ the rate of the compressed stream.

Let $x[n]$ be the original (uncompressed) signal and $\hat{x}^{\chi}[n]$ the reconstructed signal at the decoder.
The {\em normalized mean-squared error (NMSE)} in (dB) is defined  by
\bea
    \Ec^{\chi} &=&10\log_{10} \frac{\sum_{n=1}^{N}|x[n]-\hat{x}^{\chi}[n]|^2}{\sum_{n=1}^{N}x^2[n]}~~(\mbox{dB})\nn\\
    &\rightarrow& 10\log_{10} \frac{\mbbE(|x[n]-\hat{x}^{\chi}[n]|^2)}{\mbbE(|x[n]|^2)} =(\text{\rm SNR}^{\chi})^{-1}    \label{eq:NMSE}
\eea
where $N$ is the length of the data sequence, and the mean-square convergence of (\ref{eq:NMSE}) assumes regularity conditions.
Note that  $\frac{1}{\Ec^{\chi}}$  has the interpretation to be the  signal-to-reconstruction noise ratio (SNR).



For the application at hand, the data rate of the uncompressed data stream can be measured by
\begin{equation}
    R^{\text{uc}}=F_sR_Q~ \mbox{(bits/sec)}
\end{equation}
where $F_s$ represents the sampling frequency of the measured signal $x(t)$ and $R_Q$  the rate of quantization (bits/sample).
The distortion of the uncompressed scheme comes only from quantization error.  For the simple $R_Q$ bits  PCM quantization, the NMSE is approximately  by
\begin{equation}
    \Ec^{\text{uc}} \approx  -6R_Q  + 1.25~~({\rm dB}).
\end{equation}
See \cite[p. 197]{Oppenheim&Schafer:99}.

\subsection{Rate-distortion measure of  ASBC: $(\eta^{\text{ASBC}},\Ec^{\text{ASBC}})$}
We provide a characterization of the compression ratio $\eta^{\text{ASBC}}$ and the NMSE of the reconstruction $\Ec^{\text{ASBC}}$.

The data rate of the  compressed data stream by ASBC is
\begin{equation}
    R^{\text{ASBC}}= \sum_{k=1}^{K} p_k\frac{F_s}{S_k}R_k + p_e F_s R_e~ \mbox{(bits/sec)},
\end{equation}
where $F_s$   is the sampling frequency of the uncompressed data, $p_k$ the probability of $k$th subband being active, $R_k$  the rate (bits/sample) of the quantization  in  the $k$th subband, $S_k$ the down-sampling rate of $k$th subband, $p_e$ the probability that the interharmonic subband is active, and $R_e$ the rate of quantization of the  interharmonic subband.     The compression ratio of ASBC is given by
\begin{equation}
        \eta^{\text{ASBC}} = \frac{R^{\text{uc}}}{R^{\text{ASBC}}}=\left(\sum_{k=1}^{K}p_k\frac{R_k}{R_QS_k} + p_e \frac{R_e}{R_Q}\right)^{-1}.
    \label{CompressionRate}
\end{equation}
If we ignore quantization, ASBC gains via adaptively down-sampling of subband signals based on subband activity.  As an example, for the 6kHz sampling of the original signal and a harmonic subband of 6Hz bandwidth, ASBC achieves  the compression ratio $1000:1$ for that subband.


The NMSE measure $\Ec^{\text{ASBC}}$ of ASBC depends on how accurately ASBC can detect the activities of harmonic and interharmonic subbands. Assuming all harmonic subbands are active and there is no interharmonics, \ie $p_e=0$, we have $\Ec^{\text{ASBC}} \approx \Ec^{\text{uc}}$ because ASBC achieves perfect reconstruction of each harmonic signals by the Nyquist sampling theorem.  In practice, $\Ec^{\text{ASBC}} > \Ec^{\text{uc}}$ when  false negative detection occurs or when there is interharmonic signal.


\subsection{Rate-distortion measure of FFT-$(k,L)$ : $(\eta^{\text{FFT}},\Ec^{\text{FFT}})$} \label{sec:FFT}
A benchmark compression scheme is based on the fast Fourier transform (FFT), herein referred to  as FFT-$(k,L)$.  It  takes a block of $L$ data samples, computes the FFT coefficients, and keeps only the $k$ largest coefficients {$X_{j}^{(1)},\cdots,X_{j}^{(k)} $} (corresponding to the positive frequencies in the $j^{th}$ block) and masks the rest.

The compression ratio of FFT-$(k,L)$  is given by
\begin{equation}
    \eta^{\text{FFT-$(k,L)$}} = \frac{L}{k},
\end{equation}
where we ignore the $\log_2 L$ bits needed to encode the frequency locations.
The NMSE of FFT-$(k,L)$  is given by
\begin{equation}
    \Ec^{\text{FFT-$(k,L)$}} = 10\log\bigg( 1-\frac{\sum_{j=1}^{N/L}\sum_{i=1}^{k} |{X_{j}^{(i)}}|^2}{\sum_{i=1}^N |x[i]|^2}\bigg).
\end{equation}



==> Simulation.tex <==
We present numerical results in two categories using synthetic and real data. The first category is the compression of CPOW measurements, where we studied the compression of synthetic waveforms with characteristics of power system signals.  These tests allowed us to evaluate the performance of benchmark techniques under different scenarios of transient events.   We also studied the compression of real data obtained by direct sampling of voltage measurements at 6 kHz.  This was a case that the signal has significant harmonics and interharmonics.  The second category is the compression of PMU measurements, including synchrophasor measurement and frequency estimations, where both synthetic and actual PMU data were used for experiments.

ASBC was compared with four benchmark techniques:  (i) FFT described in Sec.~\ref{sec:FFT},  (ii) Multi-resolution discrete wavelet transform (DWT) using same \tcr{parameter (wavelet function, decomposition level) selection method} as in \cite{Ning&Etal:11TSG}, (iii) Compressive sampling (CS) \cite{Das&Sidhu:14TII}, and (iv) Exception compression with swing door trending compression (EC-SDT) \cite{Zhang&etal:15TPS}.    Rate-distortion curves that  plot reconstruction error against compression ratio $\eta$ are used in the compression.   We use  NMSE (dB) to measure {\em reconstruction error} for CPOW data compression  and the maximum Total Vector Error (TVE)  defined in \cite{IEEEStdC37:11} for PMU compression.




\subsection{Compressions of synthetic CPOW measurements} \label{sec:synthetic}
The purpose of this experiment was to test the performance of compression when the regular sinusoidal waveform was interrupted by episodes of transient events with signals of abnormal characteristics.   We focused on four types of event signals shown in Table~\ref{table:waveform}.
Among the set of waveforms at the event state, the amplitude modulation (AM) and frequency modulation (FM) waveforms were designed according to the requirement on performance under dynamic compliance specified by \cite{IEEEStdC37:11}.  The linear chirp waveform was used to simulate the frequency ramping events, and the interharmonic (IH) waveform modeled frequency components not in multiples of the system frequency $F_0$.



\begin{table}[h]
\renewcommand{\arraystretch}{1.3}
  \caption{Test waveforms}
    \vspace{0.5em}
    \begin{tabular}{c||c}
        \hline
         \bfseries Test cases & \bfseries Signal waveforms \\
         \hline\hline
        Normal state: & $x_N(t)= \sum_{k=0}^K  a_k \cos(2\pi60(k+1)t+\phi_k)$   \\
        ~~~$\sigma_t=0$  & \\  \hline
        Event:   &   $x^{\text{AM}}(t)=\alpha_0 +\alpha \cos(2\pi \Delta t)\cos(2\pi60t + \theta_0)$ \\
        ~~~$\sigma_t=1$           &   $x^{\text{FM}}(t)=\alpha \cos(2\pi 60t+\beta \cos(2\pi \Delta t-\pi)+\theta_0)$    \\
        &  $x^{\text{Chirp}}(t) = \alpha \cos(2\pi(59.5+\gamma t) + \theta_0)$   \\
                & $x^{\text{IH}}(t) =  \sum_{k=1}^W \alpha_k\cos(2\pi f_k t+\theta_k)$
        \\\hline
    \end{tabular}

    \vspace{0.5em}
    { Signal parameters: $\sigma_t$--the switching state, $(a_k,\phi_k)$--amplitude and phase angles of harmonics, $(\alpha_k,\beta,\gamma,\theta_k)$--transient parameters, and $f_k$--interharmonic frequencies.}
    \label{table:waveform}
\end{table}




To simulate transient events, we used a two-state Markov switching model that modulated the signal between the normal state ($\sigma_t=0$)  waveform $x^{\text{Norm}}(t)$ and the event state ($\sigma=1$) with waveforms chosen from AM, FM, chirp, and IH signals. The Markov switching process was characterized by state transition rate  $(\lambda,\mu)$ where $1/\lambda$ was the expected holding time of the normal state and $1/\mu$  the expected holding time of the event state.


\begin{figure}[h]
    \centering
    \includegraphics[width=1.6in]{figs/AMCI_0.5.eps}
    \includegraphics[width=1.6in]{figs/FMCI_0.5.eps}\\
         \includegraphics[width=3in]{figs/Max-CP-log.eps}
    \caption{{\small FM/AM parameters: $\alpha_0=1,\lambda=0.1,\mu=2$.  Top panel  NMSE with 95\% confidence interval for the AM (Left) and FM (right) events.
    No high order harmonics and interharmonics.
Bottom: the maximum reconstruction error for the FM and AM events.}}
    \label{fig:CPAM-0.5}
\end{figure}



Fig.~\ref{fig:CPAM-0.5} shows the rate-distortion curve of ASBC, FFT, and DWT techniques for the FM and AM events.  The sampling rate of the original signal was 5400 Hz.  As shown in the upper panel,   the NMSE of DWT scheme was about 30 to 40 dB higher than those of  FFT and ASBC.   Note that  DWT uses non-sinusoidal basis functions.  They tend to be effective for approximately constant or staircase valued signals (such as phasor measurements).  For the compression of sinusoidal voltage/current CPOW measurements,  sinusoidal basis functions used in ASBC and FFT had the advantage of being closer to the native voltage/current waveforms even for linear chirp signals.  In this experiment,  the requirement of high compression ratios forced DWT to discard too many parameters, resulting in high reconstruction error.

ASBC had about 4-6 dB gain over FFT for the compression ratio between 540:1 and 54:1, whereas FFT had 3 dB gain over ASBC at a compression ratio of 1350:1.  Note that the 95\% confidence interval of ASBC was considerably smaller than that of FFT, indicating that the errors of the FFT scheme were more dispersed.  The same behavior was confirmed by the maximum reconstruction error plot at the lower panel of Fig.~\ref{fig:CPAM-0.5}.    The main reason that ASBC outperformed FFT was that FFT introduced discontinuities at the boundaries of FFT blocks. In contrast, the ASBC encoder did not have discontinuities.  This phenomenon was more pronounced for the linear-chirp test cases shown in Fig.~\ref{fig:CPLC-0.5}



\begin{figure}[h]
    \centering
    \includegraphics[width=1.5in]{figs/LCCI_1.eps}
        \includegraphics[width=1.5in]{figs/LC-t-3.eps}
    \caption{{Left: comparison of rate-distortion curve for linear chip events. Right: a segment of the original and its reconstruction.  $\lambda=0.1$, $\mu=1$}}
    \label{fig:CPLC-0.5}
\end{figure}


Fig.~\ref{fig:CPLC-0.5} shows the rate-distortion plot for the linear chirp events.  The linear chirp signals have a much wider bandwidth, and the achievable compression ratio significantly lower than possible in  FM/AM events.  The left panel shows the NMSE for the three techniques.  Again, DWT was not competitive against  FFT and ASBC techniques,  and ASBC had a considerable gain over the FFT  compression in the low compression ratio regime.  In particular, ASBC had about 15 dB lower NMSE at the compression ratio of 180:1 and 20 dB lower at the compression ratio of 54:1.   The right panel shows the original signal and reconstructed ones in the time domain.  Notice that the normal sinusoidal waveform transitioned to a linear chip at time $t=16$ seconds.  The reconstruction of FFT and DWT around $t=16$  showed a significantly larger error than that of ASBC.





\subsection{Compressions of CPOW voltage measurements.}
We applied ASBC directly to a data set (hereafter referred to as UTK6K) provided by the University of Tennessee, Knoxville. The UTK6K data set consisted of 1.8 million voltage measurements sampled at 6KHz. Fig.~\ref{fig:Spectrum} (Top) shows the power spectrum of the directly sampled data stream, from which we observed the presence of harmonics and interharmonics.  The plot also showed that the energy levels from the 20th to 50th subbands were negligible.



%\begin{figure}[h]
%    \centering
%    \includegraphics[width=3.3in]{figs/UTK6k.eps}
%    \caption{Voltage Compression of 3Hz Subband Width}
%    \label{fig:UTK6KHz3}
%\end{figure}


ASBC was implemented with 3 Hz bandwidth for subbands associated with all 50 harmonics. Only the top  $k$ subbands with the highest energy level were compressed and delivered where $k$ was chosen to have the required compression ratio.  The bottom left panel of Fig.~\ref{fig:Spectrum} shows the rate-distortion curve of ASBC, FFT, and DWT for the compression ratio from 400:1 to 40:1.   For this range of compression ratios, DWT was not competitive.  ASBC was seen to out-perform FFT in the compression ratio range of 400:1 to 100:1, and the two schemes are comparable for the range of 66.7:1 to 40:1.   The reason that FFT-based compression did not perform well was, again,  that the block implementation of FFT introduced discontinuities, which caused reconstruction errors.  As the compression ratio decreased, more FFT coefficients were preserved, the reconstruction error of FFT improved.



To evaluate the effects of interharmonics, we added additional interharmonic transient events to the original UTK6KHz dataset in the same way as experiments discussed in Sec.~\ref{sec:synthetic}.  The bottom right panel of Fig.~\ref{fig:Spectrum} shows the rate-distortion plot with interharmonics subband activated. An energy detector was used to determine when and whether the interharmonics subband should be activated. Only those harmonics subbands with sufficient energy levels were compressed and transmitted. Interharmonics subband, when detected being active by the energy detector, was compressed dynamically to the effective bandwidth ranging from $60$ to $120$Hz.  As shown in the bottom left panel, the presence of interharmonics increased NMSE slightly for ASBC at the high compression ratio.  Overall, ASBC consistently performed better than other methods. The standard deviations were small for all three methods; thus, the confidence intervals were not shown in the plot.



%\begin{figure}[h]
%    \centering
%    \includegraphics[width=2.5in]{figs/InterHar.eps}
%    \caption{Rate Distortion Plot w/ Interharmonics Subband Activated}
%    \label{Fig:InterHar}
%\end{figure}



\begin{figure}[h]
    \centering
    \includegraphics[width=3in]{figs/PSD.eps}\\
    \includegraphics[width=1.6in]{figs/UTK6k.eps}
        \includegraphics[width=1.6in,height=1.3in]{figs/InterHar.eps}
    \caption{{Top: Power spectrum density of  the direct voltage measurements. Bottom left: comparison of rate-distortion curves without interharmonics. Bottom right: comparison with added interharmonics.}}
    \label{fig:Spectrum}
\end{figure}


\subsection{Compressions of PMU dynamic compliance performance}
ASBC can also be used for compressing the streaming of PMU data.  Besides  ASBC,  FFT,  and DWT compressions, we also considered two methods based on compression principles other than Fourier or wavelet-based techniques.  One technique was the application of the compressive sampling (CS) technique \cite{Das&Sidhu:14TII}; the other was based on a combination of exception compression and swing-door-trending compression (EC-SDT).  EC-SDT is a heuristic that forms a time-varying band that covers measurements and interpolating these measurements by a piecewise linear reconstruction.


\begin{figure}[h]
    \centering
    \includegraphics[width=1.65in]{figs/Max-Tve-5.eps}
            \includegraphics[width=1.65in]{figs/Synchronphasor.eps}
    \caption{Left: Max TVE fixed at compression ratio 3:1. Right: Rate distortion with $\omega=5$Hz. $k_x=0.1$, $k_a=0.1$}
    \label{fig:Synthetic-PMU}
\end{figure}


Fig.~\ref{fig:Synthetic-PMU} shows the performance of the dynamic compliance test of the benchmark techniques.  The left panel of Fig.~\ref{fig:Synthetic-PMU} shows the maximum total variation error (TVE) vs. the frequency of amplitude/phase variation at the low compression ratio\footnote{The maximum compression ratio  used in \cite{Zhang&etal:15TPS} was converted to the standard definition in (\ref{eq:CR})} of 3:1.  All tested methods except FFT satisfied the 1\% maximum TVE requirement of  IEEE C37.118.1-2011 up to 2Hz modulation frequency. FFT performed the worst for it suffered badly from the discontinuity between blocks.  The compressive sampling (CS) solution appeared to be more sensitive to the modulation frequency. Among the rest techniques, DWT performs the best at this compression ratio, and EC-SDT performed slightly better than ASBC at the lower modulation frequency. 

The right panel of Fig.~\ref{fig:Synthetic-PMU} shows the performance comparison in a  significantly higher range of compression ratios.  \tcr{ASBC, DWT and EC-SDT performed similarly up to 30:1 compression ratio, and ASBC outperformed both DWT and EC-SDT above the compression ratio of 30:1. The max TVE of FFT remains high throughout the tests due to discontinuity.}


\subsection{Compressions ov  PMU frequency measurements}
We applied ASBC to a dataset referred to as UTK1.44, which consisted of frequency estimates from the  University of Tennessee, Knoxville.  The dataset contained two data streams, each with 1,800,000 samples at the rate of 1440 samples/sec.   One distinct feature of this dataset was the frequency ramping event between 308.4 and 308.6  seconds, as shown in the right panel of  Fig.~\ref{fig:FE}.
As a time series, the frequency measurements are close to being constant at around 60 (Hz).  Thus only a single subband is needed for ASBC. We varied the subband bandwidth to achieve different compression ratios.




The performance of the four data compression methods was evaluated base on the maximum error of the reconstruction of the frequency measurements (Max FE) as  defined by the IEEE Standard C37.11  \cite{IEEEStdC37:11} that specified the acceptable performance is to have
Max-FE below 0.005 Hz.   The left panel of Fig.~\ref{fig:FE} shows the Max-FE against compression ratio.   Max-FE for DWT greatly exceeds the
IEEE Standard C37.11 standard and is not shown in the plot.  \tcr{In this case, ASBC, FFT, EC-SDT, and DWT appeared to have similar performance along the rate-distortion curve,  with DWT performing slightly better. Note that only ASBC and DWT has Max FE smaller than 0.005 Hz at compression ratio 48:1.}



\begin{figure}[h]
    \centering
   \includegraphics[width=1.6in]{figs/FE-max-1.eps}
          \includegraphics[width=1.6in]{figs/FE-t-marker-3-1.eps}
    \caption{{Maximum FE and time-domain reconstruction}}
    \label{fig:FE}
\end{figure}




\tcb{The right panel of Fig.~\ref{fig:FE} showed a segment time-domain reconstructions at the compression ratio of 48:1. For different techniques, the patterns of reconstruction error manifested themselves differently in Fig.~\ref{fig:FE}.    As Fourier based compression techniques, ASBC and FFT compression exhibited well known small but consistent sinusoidal artifacts even when the original signal was approximately constant. Such artifacts are results of the optimal sinusoidal approximation of non-sinusoidal waveforms\footnote{As suggested by the Chebyshev alternation theorem, the optimal approximation error must oscillate around the true value.}.  Because the magnitude of the errors are well within the specification of the IEEE  C37.11 Standard, such artifacts are treated as noise not to be confused by the oscillatory behavior of the system.    
 Note that the small spike of reconstruction error of FFT around $t=309$ sec.  This is caused by the discontinuity of the block implementation of FFT. } \tcr{With carefully chosen decomposition level and wavelet function, DWT performs the best among all the methods.}
 
 

\tcb{
\subsection{Implementation Issues}
We now discuss briefly implementation issues of the proposed compression technology.   As shown in Fig.~\ref{fig:encode}-\ref{fig:decode}, major costs of  implementations are the frequency up/down shifts and subband  filters in the ASBC encoder and decoder. Such operations are standard communication systems; only minor modifications of the off-the-shelf technology are necessary.   The costs of hardware implementations are extremely low.}

\tcb{The overall performance of the compression technology depends, naturally, on setting design parameters appropriately for power system signals.  This includes choosing appropriately the size of the encoding and decoding filterbank to tradeoff implementation accuracy and filtering delays.  Classical signal processing techniques such windowing offers practical ways to achieve good tradeoffs.
}

==> intro.tex <==

With deeper penetration of inverter-based resources that exhibit low inertia and fast dynamics, there are growing needs for high-resolution grid measurement and streaming technology  \cite{Liu:20Workshop,Silverstein&Follum:20NAPSI}.    In \cite{Silverstein&Follum:20NAPSI},
Silverstein and Follum make a compelling case that the time-synchronized continuous point-on-wave (CPOW) measurement technology has the potential to address operational challenges in a broad range of grid applications beyond the capabilities of the existing phasor-measurement unit (PMU) technology.  These applications include monitoring geomagnetic disturbances, subsynchronous resonance (SSR), rapid phase-jumps, and high-resolution monitoring of inverter-based distributed energy resources.   The need for high-resolution PMU data to capture new phenomenon such as super harmonics and oscillations has also been articulated in \cite{Liu:20Workshop}.

Anticipating that future wide-area measurement systems (WAMS) will likely include CPOW, PMU, and SCADA devices, this paper proposes a lossy compression technique for the high-fidelity and high-resolution streaming technology in either continuous or burst modes.  By high-fidelity, we mean that the signal reconstruction has the accuracy within specifications of the industry standard. By high-resolution, on the other hand, we mean that the source signal is sampled at sufficiently high frequencies to capture higher-order harmonics, wideband interharmonics, and wideband transients.



\begin{figure}[htb]
\begin{psfrags}
\psfrag{x}[c]{\Large $$}
\psfrag{y}[c]{\Large $$}
\psfrag{z}[c]{\Large $$}
\centerline{\scalefig{0.45}\epsfbox{figs/SamplingRates.eps}}
\end{psfrags}
\caption{Device sampling frequencies,  (uncompressed) device reporting rates for different applications and devices, and compression ratio required for streaming at the rate of 256 samples/sec. Frequency ranges are approximately illustrated. (Figure adapted from \cite{Silverstein&Follum:20NAPSI,Anderson&Agrawal&vanNess:99book,Perez:10PRE}.)}
\label{fig:sampling}
\end{figure}

CPOW technology produces time-synchronized continuous streams of direct samples of measured signals at a data rate ranging from 256 Hz to 1 MHz \cite{Silverstein&Follum:20NAPSI}.  Point-on-wave (POW) measurement devices already exist, such as digital fault and disturbance recorders (DFR/DDR). Traditionally,   high-resolution point-on-wave (POW) measurements are event-triggered designed for post-event analysis.  Fig.~\ref{fig:sampling} shows the timescales of various grid events and existing measurement devices that generate event-triggered measurements.    Also shown are the two existing streaming technologies based on SCADA\footnote{SCADA: supervisory control and data acquisition.} and PMU devices.

A critical difference between CPOW and PMU/SCADA measurements is that CPOW produces unfiltered high-resolution
voltage and current samples.  Such measurements capture crucial details in transient events that reveal operational risks.  For example, the post-event analysis of the 2016 Big Cut Fire by NERC  \cite{NERC:17} shows that the rapid voltage phase jumps caused many inverter trippings that led to the loss of 1,200 MW solar generation.  Such events would not have been observed with sufficient accuracy by traditional PMU and SCADA measurements.  NERC report concludes that  POW measurements are the most useful sources of data.

Data compression is a key technology for future high-resolution WAMS. If the existing communication infrastructure is used for streaming,
compression ratios of 100-1000 are necessary for monitoring events such as line switching voltages and some of the lightning overvoltages, as shown in Figure~\ref{fig:sampling}. Currently, there is no existing technology that provides such levels of compression.  See  \cite{Tcheou&etal:14TSG}.

Having a high compression ratio is only one measure in evaluating a compression technology.   Fundamental to streaming data compression is the tradeoff among three factors: (i) the compression ratio, (ii) the accuracy of the compression-decompression algorithm,  and (iii) the delay associated with the compression and decompression processes.  The tradeoff between the first two can be formalized in an information-theoretic setting as the {\em rate-distortion tradeoff} by Shannon \cite{Cover&Thomas:Book}.  The last is relevant in streaming applications where encoding/decoding delays are crucial constraints.






\subsection{Related Literature}
There are no compression techniques and standards for the real-time streaming of CPOW data to our best knowledge.  Here we review some of the relevant  technologies that can be candidates for high rate  CPOW/PMU data streaming.

The need for data compression for power system monitoring goes back at least three decades.  Mehta and Russell made one of the earliest contributions in \cite{Mehta&Russell:89TPD}, where they recommended compressing data in the frequency domain using the Fast Fourier Transform (FFT) by discarding high-frequency coefficients. Discarding high-frequency components may lead to significant distortions, however, when the signal has higher-order harmonics.  By processing data
 in blocks, FFT-based techniques introduce inter-block distortions.


%From an information-theoretic perspective, a modification of Mehta and Russell's suggestion by a reverse water-filling strategy can achieve the optimal tradeoff between compression ratio and reconstruction error  \cite{Cover&Thomas:Book}.  The caveat for the optimality of FFT-based compression is that the FFT block size must be large, which conflicts with the low latency requirement of data streaming.  When the FFT block size is limited, the FFT-based compression introduces inter-block distortions, resulting in the loss of signal details and high reconstruction errors.

There is an extensive  literature on compression of POW measurements  by event-triggered digital fault recorders (DFR) \cite{Littler&Morrow:99TPD,Santoso&Powers&Grady:97TPD,Gaouda&etal:00TPD,Santoso&etal:00TPD,Dash&etal:03TPD,Tse&etal:12TPD}.  For such applications, the data sampling rate can be as high as 10MHz.
Because the recorded data are used in post-event analysis, these techniques are designed to be efficient for offline storage instead of real time streaming. To this end, having accurate reconstruction is more important than having a high compression ratio and small compression/decompression delay.  Thus lossless compression techniques are often preferred.  Block linear processing techniques  such as FFT,  discrete-cosine transform (DCT), discrete wavelet transform (DWT) and spline have been developed  \cite{Mehta&Russell:89TPD,Littler&Morrow:99TPD,Santoso&Powers&Grady:97TPD,Gaouda&etal:00TPD,Santoso&etal:00TPD,Dash&etal:03TPD,Tse&etal:12TPD,Meher&Pradhan&Panda:03EPSR,Ning&Etal:11TSG}.   Nonlinear techniques such as neural network, fuzzy logic, and  principal component analysis (PCA) have also been proposed \cite{Meher&Pradhan&Panda:03EPSR,Santoso&etal:00TPD,Ibrahim&Morcos:05TPD,Ge&etal:15TSG}.

PMU data compression for efficient storage has also  attracted considerable attention \cite{Klump&etal:10PESGM,Gadde&etal:16TSG,Kummerow&Nicolai&Bretschneider:18EnergyCon}.   Such applications are significantly different from real-time streaming. It is often assumed that multiple data streams are accessible by the compression algorithm so that spatiotemporal properties can be exploited.  Two-step procedures \cite{Gadde&etal:16TSG,Kummerow&Nicolai&Bretschneider:18EnergyCon} that first compress in the spatial domain using PCA followed by temporal compression techniques (such as DCT and DWT based techniques) have shown to be effective.


The literature on the compression of streaming data for power system monitoring and control is limited.   See a survey on compression techniques for PMU data in real-time smart grid operations  \cite{Tcheou&etal:14TSG}, where the authors reported the capabilities of various compression techniques with the compression ratio up to  5:1 for lossless compressions.   Most relevant to our work are the lossy compressions, categorized by wavelet (and waveform packet) transform techniques, mixed transform, parametric and nonparametric techniques  \cite{Tcheou&etal:14TSG,Das&Sidhu:14TII,Zhang&etal:15TPS}.  These state-of-the-art methods offer a 6 to 16:1 compression ratio at the normalized mean squared error (NMSE) from -20 to -30 dB.  These techniques typically do not work well for compressing  rapid varying wideband CPOW data.

In a broader context,  the idea of subband compression considered in this paper has long been successfully applied in multimedia communications. Most of the data-streaming techniques (such as the H.264 group) employ some forms of subband compression.  The key to subband compression is to exploit the signal's subband properties to apply high levels of compression in subbands where artifacts of compression are insignificant. For instance, in audio and video compression, the audio/video signals' perceptual properties play a crucial role in achieving tradeoffs among compression ratio, reconstruction accuracy, and encoding-decoding latency.    In this paper, we focus on exploiting the harmonic structure of current/voltage signals for compression.







\subsection{Summary of Results and Contributions}  

Given that it is likely that  CPOW and PMU technologies will  coexist in a future wide-area monitoring ecosystem,  it is particularly desirable that a single compression technology applies to both data types.  To this end, the  proposed technique, referred to as {\em adaptive subband compression (ASBC)},  is perhaps the first such compression technique.
Fig.~\ref{fig:network} illustrates a conceptual infrastructure realization of the ASBC technology.
ASBC consists of an encoder for each remote sensing device and a decoder at the fusion center\footnote{A fusion center is a location where data streams from different sensing devices are combined.  A fusion center may be located at  PMU data concentrators (PDC) or the operator's control center.}.  Together, they form the ASBC codec that provides end-to-end data streaming.  Implementations of the ASBC codec are explained in Sec.~\ref{sec:encoder}-\ref{sec:decoder}.


\begin{figure}[h]
\begin{psfrags}
\psfrag{x}[c]{\Large $$}
\psfrag{y}[c]{\Large $$}
\psfrag{z}[c]{\Large $$}
\scalefig{0.5}\epsfbox{figs/network.eps}
\end{psfrags}
\caption{An application of ASBC technology for high resolution PMU monitoring of power grids.}
\label{fig:network}
\end{figure}



ASBC partitions the signal spectrum into harmonic and interharmonic subbands, as shown in Fig.~\ref{fig:Xf}.  The harmonic subbands are centered at integral multiples of the system frequency (50 or 60 Hz).  Each harmonic subband contains frequency components within the sideband of a specific bandwidth.    The interharmonic subband, on the other hand,  is a set of frequency bands between harmonic subbands \cite{Testa&etal:07TPD}.

A key feature of ASBC is adaptivity.  The encoder monitors activity of subbands and transmits only signals from active subbands.  Such an approach is instrumental when transients and interharmonics are episodic and wideband.   The level of interharmonics may be negligible most of the time and becomes strong suddenly when magnified by resonance. Thus an in-situ compression of interharmonics can achieve a high compression ratio without affecting reconstruction accuracy.

In evaluating the performance of ASBC, we provide a theoretical characterization of the compression ratio and the normalized mean-squared error (NMSE) of ASBC  and a set of numerical comparisons between ASBC and selected benchmark techniques.


Key symbols used  are listed in Table~\ref{tab:symbols}.  Otherwise, notations used in this paper are standard.  We use $x(t)$  and $x[n]$  for continuous-time and discrete-time signals, respectively.

{\small
\begin{table}[h]
\caption{\small Major symbols (in alphabetic order).}
\begin{center}
\begin{tabular}{|ll|}
\hline
$e(t)$: &noise outside harmonic subbands.\\
\hline
$F_s$: &sampling frequency of the uncompressed signal\\\hline
$p_k$: & probability of the $k$th subband being active \\
$p_e$: &probability of interharmonic subband being active\\\hline
$R_k$: & rate of quantization for the $k$th subband.\\
$R_e$: &rate of quantization for the interharmonic subband\\\hline
$S_k$:  &downsampling factor of the $k$th subband.\\\hline
$u_k[n]$: & upsampled signal from $\tilde{x}_k^Q[n]$. The data rate is the
\\& same as $y_k[n]$ \\\hline
$x(t),x[n]$: & measurement signal model.\\
$x_k(t),x_k[n]$: & signal component associated with the $k$th harmonic  \\
& with $W_k$ as its bandwidth.\\
$\tilde{x}_k[n]$: &downsampled measurements from $y_k[n]$. \\
$\tilde{x}^Q_k$: &quantized bit-stream of $\tilde{x}_k[n]$ .\\\hline
$\tilde{x}_k[n]$: &downsampled measurements from $y_k[n]$. \\\hline
$y_k[n]$: &  baseband representation of the $k$th harmonic $x_k[n]$.  \\
$\hat{y}_e[n]$: & reconstruction of the interharmonic subband signal. \\\hline
%&FFT/DWT based technique can be used for compression\\
%&of interharmonic subband.\\\hline
$\varepsilon^\chi$: & normalized mean squared error of compression\\
& technique $\chi$\\
$\eta^{\chi}$: &compression ratio of compression  technique $\chi$ \\
\hline
\end{tabular}
%\caption{\small Major symbols (in alphabetic order).}
\end{center}
\label{tab:symbols}
\end{table}
}



==> intro_v8.tex <==

With deeper penetration of inverter-based resources that exhibit low inertia and fast dynamics, there are growing needs for high-resolution grid measurement and streaming technology  \cite{Liu:20Workshop,Silverstein&Follum:20NAPSI}.    In \cite{Silverstein&Follum:20NAPSI},
Silverstein and Follum make a compelling case that the time-synchronized continuous point-on-wave (CPOW) measurement technology has the potential to address operational challenges in a broad range of grid applications beyond the capabilities of the existing phasor-measurement unit (PMU) technology.  These applications include monitoring geomagnetic disturbances, subsynchronous resonance (SSR), rapid phase-jumps, and high-resolution monitoring of inverter-based distributed energy resources.   The need for high-resolution PMU data to capture new phenomenon such as super harmonics and oscillations has also been articulated in \cite{Liu:20Workshop}.

Anticipating that future wide-area measurement systems (WAMS) will likely include CPOW, PMU, and SCADA devices, this paper proposes a lossy compression technique for the high-fidelity and high-resolution streaming technology in either continuous or burst modes.  By high-fidelity, we mean that the signal reconstruction has a low compression reconstruction error within industry standards specification. By high-resolution, on the other hand, we mean that the source signal is sampled at sufficiently high frequencies to capture higher-order harmonics, wideband interharmonics, and wideband transients.



\begin{figure}[htb]
\begin{psfrags}
\psfrag{x}[c]{\Large $$}
\psfrag{y}[c]{\Large $$}
\psfrag{z}[c]{\Large $$}
\centerline{\scalefig{0.45}\epsfbox{figs/SamplingRates.eps}}
\end{psfrags}
\caption{Device sampling frequencies,  (uncompressed) device reporting rates for different applications and devices, and compression ratio required for streaming at the rate of 256 samples/sec. Frequency ranges are approximately illustrated. (Figure adapted from \cite{Silverstein&Follum:20NAPSI,Anderson&Agrawal&vanNess:99book,Perez:10PRE}.)}
\label{fig:sampling}
\end{figure}

CPOW technology produces time-synchronized continuous streams of direct samples of measured signals at a data rate ranging from 256 Hz to 1 MHz \cite{Silverstein&Follum:20NAPSI}.  Point-on-wave (POW) measurement devices already exist, such as digital fault and disturbance recorders (DFR/DDR). Traditionally,   high-resolution point-on-wave (POW) measurements are event-triggered designed for post-event analysis.  Fig.~\ref{fig:sampling} shows the timescales of various grid events and existing measurement devices that generate event-triggered measurements.    Also shown are the two existing streaming technologies based on SCADA\footnote{SCADA: supervisory control and data acquisition.} and PMU devices.

A critical difference between CPOW and PMU/SCADA measurements is that CPOW produces unfiltered high-resolution
voltage and current samples.  Such measurements capture crucial details in transient events that reveal operational risks.  For example, the post-event analysis of the 2016 Big Cut Fire by NERC  \cite{NERC:17} shows that the rapid voltage phase jumps caused many inverter trippings that led to the loss of 1,200 MW solar generation.  Such events would not have been observed with sufficient accuracy by traditional PMU and SCADA measurements.  NERC report concludes that  POW measurements are the most useful sources of data.

Data compression is a key technology for future high-resolution WAMS. If the existing communication infrastructure is used for streaming,
compression ratios of 100-1000 are necessary for monitoring events such as line switching voltages and some of the lightning overvoltages, as shown in Figure~\ref{fig:sampling}. Currently, there is no existing technology that provides such levels of compression.  See  \cite{Tcheou&etal:14TSG}.

Having a high compression ratio is only one measure in evaluating a compression technology.   Fundamental to streaming data compression is the tradeoff among three factors: (i) the compression ratio, (ii) the accuracy of the compression-decompression algorithm,  and (iii) the delay associated with the compression and decompression processes.  The tradeoff between the first two can be formalized in an information-theoretic setting as the {\em rate-distortion tradeoff} by Shannon \cite{Cover&Thomas:Book}.  The last is relevant in streaming applications where encoding/decoding delays are crucial constraints.






\subsection{Related Literature}
There are no compression techniques and standards for the real-time streaming of CPOW data to our best knowledge.  Here we review some of the relevant  technologies that can be candidates for high rate  CPOW/PMU data streaming.

The need for data compression for power system monitoring goes back at least three decades.  Mehta and Russell made one of the earliest contributions in \cite{Mehta&Russell:89TPD}, where they recommended compressing data in the frequency domain using the Fast Fourier Transform (FFT) by discarding high-frequency coefficients. Discarding high-frequency components may lead to significant distortions, however, when the signal has higher-order harmonics.  By processing data
 in blocks, FFT-based techniques introduce inter-block distortions.


%From an information-theoretic perspective, a modification of Mehta and Russell's suggestion by a reverse water-filling strategy can achieve the optimal tradeoff between compression ratio and reconstruction error  \cite{Cover&Thomas:Book}.  The caveat for the optimality of FFT-based compression is that the FFT block size must be large, which conflicts with the low latency requirement of data streaming.  When the FFT block size is limited, the FFT-based compression introduces inter-block distortions, resulting in the loss of signal details and high reconstruction errors.

There is an extensive  literature on compression of POW measurements  by event-triggered digital fault recorders (DFR) \cite{Littler&Morrow:99TPD,Santoso&Powers&Grady:97TPD,Gaouda&etal:00TPD,Santoso&etal:00TPD,Dash&etal:03TPD,Tse&etal:12TPD}.  For such applications, the data sampling rate can be as high as 10MHz.
Because the recorded data are used in post-event analysis, these techniques are designed to be efficient for offline storage instead of real time streaming. To this end, having accurate reconstruction is more important than having a high compression ratio and small compression/decompression delay.  Thus lossless compression techniques are often preferred.  Block linear processing techniques  such as FFT,  discrete-cosine transform (DCT), discrete wavelet transform (DWT) and spline have been developed  \cite{Mehta&Russell:89TPD,Littler&Morrow:99TPD,Santoso&Powers&Grady:97TPD,Gaouda&etal:00TPD,Santoso&etal:00TPD,Dash&etal:03TPD,Tse&etal:12TPD,Meher&Pradhan&Panda:03EPSR,Ning&Etal:11TSG}.   Nonlinear techniques such as neural network, fuzzy logic, and  principal component analysis (PCA) have also been proposed \cite{Meher&Pradhan&Panda:03EPSR,Santoso&etal:00TPD,Ibrahim&Morcos:05TPD,Ge&etal:15TSG}.

PMU data compression for efficient storage has also  attracted considerable attention \cite{Klump&etal:10PESGM,Gadde&etal:16TSG,Kummerow&Nicolai&Bretschneider:18EnergyCon}.   Such applications are significantly different from real-time streaming. It is often assumed that multiple data streams are accessible by the compression algorithm so that spatiotemporal properties can be exploited.  Two-step procedures \cite{Gadde&etal:16TSG,Kummerow&Nicolai&Bretschneider:18EnergyCon} that first compress in the spatial domain using PCA followed by temporal compression techniques (such as DCT and DWT based techniques) have shown to be effective.


The literature on the compression of streaming data for power system monitoring and control is limited.   See a survey on compression techniques for PMU data in real-time smart grid operations  \cite{Tcheou&etal:14TSG}, where the authors reported the capabilities of various compression techniques with the compression ratio up to  5:1 for lossless compressions.   Most relevant to our work are the lossy compressions, categorized by wavelet (and waveform packet) transform techniques, mixed transform, parametric and nonparametric techniques  \cite{Tcheou&etal:14TSG,Das&Sidhu:14TII,Zhang&etal:15TPS}.  These state-of-the-art methods offer a 6 to 16:1 compression ratio at the normalized mean squared error (NMSE) from -20 to -30 dB.  These techniques typically do not work well for compressing  rapid varying wideband CPOW data.

In a broader context,  the idea of subband compression considered in this paper has long been successfully applied in multimedia communications. Most of the data-streaming techniques (such as the H.264 group) employ some forms of subband compression.  The key to subband compression is to exploit the signal's subband properties to apply high levels of compression in subbands where artifacts of compression are insignificant. For instance, in audio and video compression, the audio/video signals' perceptual properties play a crucial role in achieving tradeoffs among compression ratio, reconstruction accuracy, and encoding-decoding latency.    In this paper, we focus on exploiting the harmonic structure of current/voltage signals for compression.







\subsection{Summary of Results and Contributions}
The proposed technique, referred to as {\em adaptive subband compression (ASBC)},  is perhaps the first compression technique designed to stream the CPOW (and PMU) data.  Fig.~\ref{fig:network} illustrates a conceptual infrastructure realization of the ASBC technology.
ASBC consists of an encoder for each remote sensing device and a decoder at the fusion center\footnote{A fusion center is a location where data streams from different sensing devices are combined.  A fusion center may be located at  PMU data concentrators (PDC) or the operator's control center.}.  Together, they form the ASBC codec that provides end-to-end data streaming.  Implementations of the ASBC codec are explained in Sec.~\ref{sec:encoder}-\ref{sec:decoder}.


\begin{figure}[h]
\begin{psfrags}
\psfrag{x}[c]{\Large $$}
\psfrag{y}[c]{\Large $$}
\psfrag{z}[c]{\Large $$}
\scalefig{0.5}\epsfbox{figs/network.eps}
\end{psfrags}
\caption{An application of ASBC technology for high resolution PMU monitoring of power grids.}
\label{fig:network}
\end{figure}



ASBC partitions the signal spectrum into harmonic and interharmonic subbands, as shown in Fig.~\ref{fig:Xf}.  The harmonic subbands are centered at integral multiples of the system frequency (50 or 60 Hz).  Each harmonic subband contains frequency components within the sideband of a specific bandwidth.    The interharmonic subband, on the other hand,  is a set of frequency bands between harmonic subbands \cite{Testa&etal:07TPD}.

A key feature of ASBC is adaptivity.  The encoder monitors activity of subbands and transmits only signals from active subbands.  Such an approach is instrumental when transients and interharmonics are episodic and wideband.   The level of interharmonics may be negligible most of the time and becomes strong suddenly when magnified by resonance. Thus an in-situ compression of interharmonics can achieve a high compression ratio without affecting reconstruction accuracy.

In evaluating the performance of ASBC, we provide a theoretical characterization of the compression ratio and the normalized mean-squared error (NMSE) of ASBC  and a set of numerical comparisons between ASBC and selected benchmark techniques.


Key symbols used in the paper are listed in Table~\ref{tab:symbols}.  Otherwise, notations used in this paper are standard.  We use $x(t)$ to denote a continuous-time signal and $x[n]$ a discrete-time sequence.

{\small
\begin{table}[h]
\caption{\small Major symbols (in alphabetic order).}
\begin{center}
\begin{tabular}{|ll|}
\hline
$e(t)$: &noise outside harmonic subbands.\\
\hline
$F_s$: &sampling frequency of the uncompressed signal\\\hline
$p_k$: & probability of the $k$th subband being active \\
$p_e$: &probability of interharmonic subband being active\\\hline
$R_k$: & rate of quantization for the $k$th subband.\\
$R_e$: &rate of quantization for the interharmonic subband\\\hline
$S_k$:  &downsampling factor of the $k$th subband.\\\hline
$u_k[n]$: & upsampled signal from $\tilde{x}_k^Q[n]$. The data rate is the
\\& same as $y_k[n]$ \\\hline
$x(t),x[n]$: & measurement signal model.\\
$x_k(t),x_k[n]$: & signal component associated with the $k$th harmonic  \\
& with $W_k$ as its bandwidth.\\
$\tilde{x}_k[n]$: &downsampled measurements from $y_k[n]$. \\
$\tilde{x}^Q_k$: &quantized bit-stream of $\tilde{x}_k[n]$ .\\\hline
$y_k[n]$: &  baseband representation of the $k$th harmonic $x_k[n]$.  \\
$\hat{y}_e[n]$: & reconstruction of the interharmonic subband signal. \\\hline
%&FFT/DWT based technique can be used for compression\\
%&of interharmonic subband.\\\hline
$\varepsilon^\chi$: & normalized mean squared error of compression\\
& technique $\chi$\\
$\eta^{\chi}$: &compression ratio of compression  technique $\chi$ \\
\hline
\end{tabular}
%\caption{\small Major symbols (in alphabetic order).}
\end{center}
\label{tab:symbols}
\end{table}
}


